On the Statistical Consistency of Risk-Sensitive Bayesian Decision-Making

We study data-driven decision-making problems in the Bayesian framework, where the expectation in the Bayes risk is replaced by a risk-sensitive entropic risk measure. We focus on problems where calculating the posterior distribution is intractable, a typical situation in modern applications with large datasets and complex data generating models. We leverage a dual representation of the entropic risk measure to introduce a novel risk-sensitive variational Bayesian (RSVB) framework for jointly computing a risk-sensitive posterior approximation and the corresponding decision rule. The proposed RSVB framework can be used to extract computational methods for doing risk-sensitive approximate Bayesian inference. We show that our general framework includes two well-known computational methods for doing approximate Bayesian inference viz. naive VB and loss-calibrated VB. We also study the impact of these computational approximations on the predictive performance of the inferred decision rules and values. We compute the convergence rates of the RSVB approximate posterior and also of the corresponding optimal value and decision rules. We illustrate our theoretical findings in both parametric and nonparametric settings with the help of three examples: the single and multi-product newsvendor model and Gaussian process classification.

==> Figures/EC.tex <==
%% Here starts the e-companion (EC)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Appendix}

\subsection{Alternative derivation of LCVB}
We present the alternative derivation of LCVB. Consider the logarithm of the Bayes posterior risk,
	\begin{align}
	\nonumber
	\log \mathbb{E}_{\Pi(\theta|\nX)}[\exp(R(a,\theta))]&= \log \int_{\Theta}
	\exp(R(a,\theta))
	d\Pi(\theta|\nX)\\
	\nonumber
	&=  \log \int_{\Theta} \frac{dQ(\theta)}{dQ(\theta)} \exp(R(a,\theta))
	d\Pi(\theta| \nX) \\
	\label{eq:6}
	&\geq - \int_{\Theta} dQ(\theta)\log \frac{dQ(\theta)}{\exp(R(a,\theta))
		d\Pi(\theta| \nX)} =:  \mathcal{F}(a;Q(\cdot), \nX)
	\end{align}
where the inequality follows from an application of Jensen's inequality (since, without loss of generality, $\exp(R(a,\theta)) > 0$ for all $a \in \sA$ and $\theta \in \Theta$), and $Q \in \sQ$. Then, it follows that
\begin{align}
	\nonumber
	\min_{a \in \sA} \log \mathbb{E}_{\Pi(\theta|\nX)}[\exp(R(a,\theta))]
	&\geq  \underset{a \in \sA}{\min}~\underset{q \in \mathcal{Q}}{\max}\
	\mathcal{F}(a;Q(\theta),\nX)\\
	\label{eq:reg-form2}
	&= \underset{a\in\sA}{\min}~\underset{q \in \mathcal{Q}}{\max}
	- \scKL\left(Q(\theta)|| \Pi(\theta|\nX)\right) + \int_{\Theta} 
	R(a,\theta) dQ(\theta).
	\end{align}



\subsection{Proof of Theorem~\ref{thrm:thm1}:}
We prove our main result after series of important lemmas. 
\begin{lemma}\label{lem:lem1}
	For any $a' \in \sA$, $\gamma>0$, and $\zeta>0$,
    % $\zeta:\bbR^+\mapsto \bbR^+$, 
	\begin{align}
		\nonumber
		\bbE_{P^{n}_0}& \left[ \zeta  \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right]  
		\\
		\nonumber
		\leq & \log  \bbE_{P^{n}_0} \left[ \int_{\Theta}  e^{  \zeta  L_n(\theta,\theta_0)} \frac {e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }   \right] +  \inf_{Q \in \sQ} \bbE_{P^{n}_0} \bigg[  \scKL(Q(\theta)\|\Pi(\theta|\nX))
		\\
		& - \gamma \inf_{a \in  \mathcal{A}} \bbE_Q[R(a,\theta)] \bigg]  +\log  \bbE_{P^{n}_0} \left[ \int_{\Theta} e^{\gamma R(a',\theta)} \ \frac{\prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)}{\int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)}  \right] .
		\label{eq:eqf2} 
	\end{align} 
\end{lemma}
\begin{proof}
For any fixed $a' \in \sA, \gamma > 0$, and $\zeta>0$,
% and $C(\gamma):\bbR^+\mapsto \bbR^+$, 
and using the fact that $\scKL$ is non-negative, observe that the  integral in the LHS of equation~\eqref{eq:eqf2} satisfies, 	
\begin{align}
	\nonumber
	\zeta \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs  & \leq  \int_{\Theta}  \log e^{ \zeta L_n(\theta,\theta_0)} \ d\qrs \ 
	\\
	\nonumber
	& \quad + \scKL\left( d\qrs \bigg \|\frac{e^{\zeta L_n(\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ d\Pi(\theta|\nX)}{\int_{\Theta}  e^{\zeta L_n(\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ d \Pi(\theta|\nX) } \right)
	\\
	\nonumber
	=  \int_{\Theta}  \log & e^{ \zeta L_n(\theta,\theta_0)} \ d\qrs \ + \log \int_{\Theta}  e^{ \zeta L_n(\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ d \Pi(\theta|\nX) 
	\\
	\nonumber 
	& +  \int_{\Theta}  	d\qrs  \log \frac{d\qrs}{ e^{\zeta L_n  (\theta,\theta_0)}  e^{\gamma R(a',\theta)} \ d\Pi(\theta|\nX)  }  
	\\
	\nonumber
	=  \log \int_{\Theta} & e^{ \zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ d \Pi(\theta|\nX)  +   \int_{\Theta}  	d\qrs  \log \frac{d\qrs}{e^{\gamma R(a',\theta)} \ d\Pi(\theta|\nX)  } .
\end{align}
%\prateek{1. Even if $R(a',\theta)$ is bounded from above and below, the bound above is loose. To see this, let $R(a',\theta) \in (B_1,B_2)$ and  observe that
%$\log \int_{\Theta}  e^{ \zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ d \Pi(\theta|\nX)  +  \int_{\Theta}  	\qrs  \log \frac{\qrs}{e^{\gamma R(a',\theta)} \ \Pi(\theta|\nX)  } d\theta \leq \log \int_{\Theta}  e^{ \zeta L_n  (\theta,\theta_0)}   \ d \Pi(\theta|\nX)  +  \int_{\Theta}  	\qrs  \log \frac{\qrs}{ \ \Pi(\theta|\nX)  } d\theta + \gamma(B_2-B_1)$. Moreover, if we assume that $\qrs$ concentrates as $\gamma$ increases then, $\int\qrs \log d\qrs$ increases with $\gamma$.  }

%
%\prateek{\textbf{Idea 1:}
%    \begin{align}
%        \nonumber
%        \beta \int_{\Theta}&  L_n(\theta,\theta_0)\ d\qrs  
%        \\
%        & \leq  \int_{\Theta}  \log e^{ \zeta L_n  (\theta,\theta_0)} \ d\qrs \ 
%        \\
%        \nonumber
%        & \quad + \scKL\left( \qrs \bigg \|\frac{e^{\zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)} \textcolor{red}{\mathcal{N}(\theta|\gamma,\frac{1}{\gamma})}  \ \Pi(\theta|\nX)}{\int_{\Theta}  e^{\zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)} \textcolor{red}{\mathcal{N}(\theta|\gamma,\frac{1}{\gamma})} \ d \Pi(\theta|\nX) } \right)
%        \\
%        \nonumber
%        &= \log \int_{\Theta}  e^{ \zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)} \textcolor{red}{  e^{-\frac{\gamma}{2}(\theta-\gamma)^2}} \ d \Pi(\theta|\nX)  +  \int_{\Theta}  	\qrs  \log \frac{\qrs}{e^{\gamma R(a',\theta)} \ \Pi(\theta|\nX)  } d\theta
%        \\
%        \nonumber
%        &\quad -   \int_{\Theta}  	\qrs  \log \textcolor{red}{  e^{-\frac{\gamma}{2}(\theta-\gamma)^2}}d\theta.
%        \end{align}
%}
%
%\prateek{\textbf{Idea 3:}
%    \begin{align}
%        \nonumber
%        \beta \int_{\Theta}&  L_n(\theta,\theta_0)\ d\qrs  
%        \\
%        & \leq  \int_{\Theta}  \log e^{ \zeta L_n  (\theta,\theta_0)} \ d\qrs \ 
%        \\
%        \nonumber
%        & \quad + \frac{1}{C(\gamma)}\scKL\left( \qrs \bigg \|\frac{e^{C(\gamma) \zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ \Pi(\theta|\nX)}{\int_{\Theta}  e^{C(\gamma) \zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ d \Pi(\theta|\nX) } \right)
%        \\
%        \nonumber
%        &= \frac{1}{C(\gamma)}\log \int_{\Theta}  e^{ C(\gamma) \zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ d \Pi(\theta|\nX)  + \frac{1}{C(\gamma)} \int_{\Theta}  	\qrs  \log \frac{\qrs}{e^{\gamma R(a',\theta)} \ \Pi(\theta|\nX)  } d\theta
%        %\\
%        %\nonumber
%        %&\quad -   \int_{\Theta}  	\qrs  \log \textcolor{red}{  e^{-\frac{\gamma}{2}(\theta-\gamma)^2}}d\theta.
%    \end{align}
%}


%\prateek{\textbf{Idea 2:}
%    \begin{align}
%        \nonumber
%        \beta \int_{\Theta}&  L_n(\theta,\theta_0)\ d\qrs  
%        \\
%        & \leq  \int_{\Theta}  \log e^{ \zeta L_n  (\theta,\theta_0)} \ d\qrs \ 
%        \\
%        \nonumber
%        & \quad + \scKL\left( \qrs \bigg \|\frac{e^{\zeta L_n  (\theta,\theta_0)} e^{\frac{\gamma}{\textcolor{red}{C(\gamma)}} R(a',\theta)}   \ \Pi(\theta|\nX)}{\int_{\Theta}  e^{\zeta L_n  (\theta,\theta_0)} e^{\frac{\gamma}{\textcolor{red}{C(\gamma)}} R(a',\theta)} \ d \Pi(\theta|\nX) } \right)
%        \\
%        \nonumber
%        &= \log \int_{\Theta}  e^{ \zeta L_n  (\theta,\theta_0)} e^{\frac{\gamma}{\textcolor{red}{C(\gamma)}} R(a',\theta)} \ d \Pi(\theta|\nX)  +  \int_{\Theta}  	\qrs  \log \frac{\qrs}{e^{\frac{\gamma}{\textcolor{red}{C(\gamma)}} R(a',\theta)} \ \Pi(\theta|\nX)  } d\theta
%        \\
%        \nonumber
%        &= \log \int_{\Theta}  e^{ \zeta L_n  (\theta,\theta_0)} e^{\frac{\gamma}{\textcolor{red}{C(\gamma)}} R(a',\theta)} \ d \Pi(\theta|\nX)  +  \int_{\Theta}  	\qrs  \log \frac{\qrs}{ \ \Pi(\theta|\nX)  } d\theta
%        \\
%        &\quad - \frac{\gamma}{\textcolor{red}{C(\gamma)}} \int_{\Theta} \qrs  R(a',\theta) d\theta
%    \end{align}
%}
Next, using the definition of $\qrs$ in the second term of last equality, for any other $Q(\cdot) \in \sQ$
\begin{align}
	\nonumber
	\zeta \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs  \leq \log \int_{\Theta}  &e^{\zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ d \Pi(\theta|\nX)  +  \int_{\Theta}  	dQ(\theta)  \log \frac{dQ(\theta)} {e^{\gamma R(a',\theta)} \ d\Pi(\theta|\nX)  } .
\end{align}
Finally, it follows from the definition of the posterior distribution that
\begin{align} 
	\nonumber
	\zeta \int_{\Theta}  & L_n(\theta,\theta_0)\ d\qrs  
	\\
	\nonumber 
	&\leq \log \int_{\Theta}   e^{\zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ \frac {\prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }   +  \int_{\Theta}  	dQ(\theta)  \log \frac{dQ(\theta)} {e^{\gamma R(a',\theta)} \ d\Pi(\theta|\nX)  } ,
	\\
	\nonumber
	=&  \log \int_{\Theta}  e^{\zeta L_n  (\theta,\theta_0)}   \ \frac { e^{\gamma R(a',\theta)} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }   +  \int_{\Theta}  	dQ(\theta)  \log \frac{dQ(\theta)} {e^{\gamma R(a',\theta)} \ d\Pi(\theta|\nX) } 
	\\
	&+ \log \int_{\Theta}  \  e^{\gamma R(a',\theta)}  \frac{\prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)}{\int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)}  , 
	\label{eq:eqf1} 
\end{align}

where the last equality follows from adding and subtracting $ \log  \int_{\Theta} e^{\gamma R(a',\theta)}  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) $. Now taking expectation on either side of equation~\eqref{eq:eqf1} and using Jensen's inequality on the first and the last term in the RHS yields
\begin{align}
	\nonumber
	\bbE_{P^{n}_0}& \left[ \zeta \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right]  
	\\
	\nonumber
	\leq  &\log  \bbE_{P^{n}_0} \left[ \int_{\Theta}  e^{\zeta L_n  (\theta,\theta_0)} \frac {e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }   \right] +  \inf_{Q \in \sQ} \bbE_{P^{n}_0} \bigg[  \int_{\Theta}   	dQ(\theta)  \log \frac{dQ(\theta)}   {d\Pi(\theta|\nX)  }  
	\\ 
	& - \gamma \inf_{a \in  \mathcal{A}} \int_{\Theta}  Q(\theta) { R(a,\theta)}	 d\theta \bigg] +\log  \bbE_{P^{n}_0} \left[ \int_{\Theta} e^{\gamma R(a',\theta)}  \ \frac{\prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)}{\int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)} \right],
	%- \bbE_{P^{n}_0} \left[ \log \int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) \right]
	%\\
	%\nonumber
	%= & \log  \bbE_{P^{n}_0} \left[ \int_{\Theta}  e^{ \zeta L_n  (\theta,\theta_0)} \frac {e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  d\theta \right] +  \inf_{Q \in \sQ} \bbE_{P^{n}_0} \bigg[  \scKL(Q(\theta)\|\Pi(\theta|\nX))
	%\\
	%& - \gamma \inf_{a \in  \mathcal{A}} \bbE_Q[R(a,\theta)] \bigg]  +\log  \bbE_{P^{n}_0} \left[ \int_{\Theta} e^{\gamma R(a',\theta)}  \ \frac{\prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \Pi(\theta)}{\int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)} d\theta \right] ,
	%- \bbE_{P^{n}_0} \left[ \log \int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) \right]
	%\label{eq:eqf2} 
\end{align}
where in the second term in RHS of~\eqref{eq:eqf1}, we first take infimum over all $a\in \sA$ which upper  bounds the second term in~\eqref{eq:eqf1} and then take infimum over all $Q \in \sQ$, since the LHS does not depend on $Q$. 
\end{proof}

Next, we state a technical result that is important  in proving our next lemma.
\begin{lemma}[Lemma 6.4 of \cite{Zhang2018}]\label{lem:lem6.4}
	Suppose random variable X satisfies
	\vspace{0em}
	$$\mathbb{P}(X\geq t) \leq c_1 \exp(-c_2 t),$$
	for all $t \geq t_0>0$. Then for any $0< \beta \leq c_2/2 $,
	$$ \bbE[ \exp(\beta X)] \leq \exp(\beta t_0) + c_1.$$
\end{lemma}
\begin{proof}
    Refer Lemma 6.4 of \cite{Zhang2018}.
    
\end{proof}
\prateek{If we assume that R is bounded utility with bound as $U_b$, then
    \begin{align} 
        \nonumber
        \zeta \int_{\Theta}  & L_n(\theta,\theta_0)\ d\qrs  
        \\
        \nonumber 
        &\leq \log \int_{\Theta}   e^{\zeta L_n  (\theta,\theta_0)} e^{\gamma R(a',\theta)}  \ \frac {\prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \Pi(\theta) } {\int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } d\theta  +  \int_{\Theta}  	dQ(\theta)  \log \frac{dQ(\theta)} {e^{\gamma R(a',\theta)} \ d\Pi(\theta|\nX)  } ,
        \\
        &\leq \log \int_{\Theta}   e^{\zeta L_n  (\theta,\theta_0)}   \ \frac {\prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \Pi(\theta) } {\int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } d\theta  +  \int_{\Theta}  	Q(\theta)  \log \frac{Q(\theta)} {\Pi(\theta|\nX)  } d\theta,
        \\
        \nonumber
        &\quad + \textcolor{red}{\gamma  \left(U_b- \int_{\Theta} Q(\theta) R(a',\theta)d\theta \right)}.
    \end{align}
    \begin{align}
        \nonumber
        \bbE_{P^{n}_0}& \left[ \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right]  \\
        \nonumber
        & \leq \frac{1}{\zeta} \left\{ \log(e^{\zeta C_{1}n \e_n^2} + (1+C_0+ 3W^{-\gamma}))  + \log \left( e^{C_{4}(\gamma) n \e_n^2} + 2C_4(\gamma) \right)  + n \eta_n^R(\gamma)  \right\}
        \\
        %\nonumber
        %& \leq (C_{1} + \frac{\omega}{\beta} C_4(\gamma) )n \e_n^2 + \frac{1}{\beta}n \eta_n^R^2(a) + \frac{(1+C_0+ 3W^{-\gamma})e^{(-\beta C_{1}n \e_n^2)}  }{\beta} 
        %\\
        \nonumber
        & \leq  C_{1}  n \e_n^2  + \frac{ \inf_{Q \in \sQ} \bbE_{P_0^n}[\int_{\Theta}  	Q(\theta)  \log \frac{Q(\theta)} {\Pi(\theta|\nX)  } d\theta  + \textcolor{red}{\gamma  \left(U_b- \int_{\Theta} Q(\theta) R(a',\theta)d\theta \right)}   ]}{\zeta} +\frac{(1+C_0)e^{(-\zeta C_{1}n \e_n^2)}   }{\zeta},
    \end{align}
}



In the following result, we bound the first term on the RHS of equation~\eqref{eq:eqf2}.
\begin{lemma}\label{lem:lem2}
	Under Assumptions~\ref{assump:Asf1},~\ref{assump:Asf2},~\ref{assump:Asf3},~\ref{assump:Asf14}, and~\ref{assump:Asf15}  and for $\min(C,C_4(\gamma) + C_5(\gamma)) > C_2 + C_3 + C_4(\gamma) + 2$ and any $\e \geq \e_n$,
	\begin{align}
		\bbE_{P^{n}_0} \left[ \int_{\Theta}  e^{\zeta L_n  (\theta,\theta_0)} \frac {e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)} {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }   \right]	\leq e^{\zeta C_{1}n \e^2} + (1+C_0+ 3W^{-\gamma}), \label{eq:eqf6}
	\end{align}
	for $0< \zeta \leq C_{10}/2 $, where $C_{10} = \min \{\lambda,C, 1\}/ C_1$ for any $\lambda>0$.
\end{lemma}
\begin{proof}
First define the set
\begin{align}
	%K_n &: = \{ \theta: L_n(\theta,\theta_0) > C_1n\e_n^2  \} \\ %\quad \forall k \in \mathbb{N}, \\
	B_n &: = \left\{\nX : \int_{\Theta}  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) \geq e^{-(1+C_3)n\e^2}\Pi(A_n) \right\} \label{def:def1},
	%\geq e^{-(1+C_3+C_2 )n\e_n^2}
	%	B_n &: = \{\nX : \int_{\Theta} e^{\gamma R(a',\theta)} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) \geq e^{(-2+C_8) n\e_n^2}\Pi(A_n) \geq e^{-(2+C_2 - C_8 )n\e_n^2}  \}
\end{align}
where set $A_n$ is  defined in Assumption~\ref{assump:Asf3}.
We demonstrate that, under Assumption~\ref{assump:Asf3}, $P^n_0 \left({B_n^c} \right)$ is bounded above by an exponentially  decreasing(in $n$) term. Note that for $A_n$ as defined in Assumption~\ref{assump:Asf3}:
\begin{align}
	\nonumber
	\mathbb P^n_0&\left( \frac{1}{\Pi(A_n)} \int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) \leq e^{-(1+C_3) n\e^2}   \right) 
	\\
	& \leq \mathbb P^n_0\left(\frac{1}{\Pi(A_n)} \int_{\Theta \cap A_n} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) \leq e^{-(1+C_3) n\e^2}   \right).  \label{eq:lc1}
\end{align}
Let $d \tilde \Pi(\theta) : = \frac{ \mathbbm{1}_{ \{\Theta \cap A_n \} }(\theta) }{\Pi(A_n)} d\Pi(\theta), $ and use this in~\eqref{eq:lc1} for any $\lambda>0$ to obtain, 
\begin{align*}
	\mathbb P^n_0\left(  \frac{1}{\Pi(A_n)} \int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) \leq e^{-(1+C_3) n\e^2} \right) & \leq \mathbb P^n_0\left(  \int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d \tilde \Pi(\theta) \leq e^{-(1+C_3) n\e^2}  \right) 
	\\
	&= \mathbb P^n_0 \left( \left[ \int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d \tilde \Pi(\theta) \right]^{-\lambda} \geq e^{ (1 + C_3) \lambda n\e^2}   \right).
\end{align*}
{Then, using the  Chernoff's inequality in the last equality above, we have  }
\begin{align}
	\nonumber
	\mathbb P^n_0\left(  \frac{1}{\Pi(A_n)} \int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) \leq e^{-(1+C_3) n\e^2} \right)
	&\leq e^{- (1+C_3) \lambda n\e^2} \bbE_{P^{n}_0} \left( \left[ \int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d \tilde \Pi(\theta) \right]^{-\lambda}    \right)
	\\
	\nonumber
	&\leq e^{- (1+C_3) \lambda n\e^2}  \left[ \int_{\Theta} \bbE_{P^{n}_0} \left( \left[ \prod_{i=1}^n \frac {p(X_i|\theta)} {p(X_i|\theta_0)} \right]^{-\lambda} \right) d \tilde \Pi(\theta) \right]    
	\\
	\nonumber
	&=  e^{- (1+C_3) \lambda n\e^2}  \left[ \int_{\Theta} \exp( \lambda D_{\lambda+1}\left( P_0^n \| P_{\theta}^n \right) ) d \tilde \Pi(\theta) \right]    
	\\
	&\leq e^{- (1+C_3) \lambda n\e^2} e^{\lambda C_3 n\e_n^2 } \leq \e^{- \lambda n \e^2}, \label{eq:eq_bn} 
\end{align}
where the second inequality follows from first applying Jensen's inequality (on the term inside $[\cdot]$) and then using Fubini's theorem, and the penultimate inequality follows from Assumption~\ref{assump:Asf3} and the definition of $\tilde \Pi(\theta)$. 

Next, define the set $K_n : = \{ \theta \in \Theta: L_n(\theta,\theta_0) > C_1n\e^2  \} $. Notice that set $K_n$ is the set of alternate hypothesis as defined in Assumption~\ref{assump:Asf1}. We bound the calibrated posterior probability of this set $K_n$ to get a bound on the first term in the RHS of equation~\eqref{eq:eqf2}. Recall the sequence of test function $\{\phi_{n,\e}\}$ from Assumption~\ref{assump:Asf1}. Observe that
\begin{align}
	\nonumber
	\bbE_{P^{n}_0} &\left[  \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] 
	\\
	\nonumber
	&= \bbE_{P^{n}_0} \left[ (\phi_{n,\e})  \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] +  \bbE_{P^{n}_0} \left[ (1 - \phi_{n,\e})  \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right]
	\\
	\nonumber
	& \leq \bbE_{P^{n}_0}  \phi_{n,\e} 
	+ \bbE_{P^{n}_0} \left[ (1 - \phi_{n,\e}) \mathbbm{1}_{B_n^C}  \right] 
	+ \bbE_{P^{n}_0} \left[ (1 - \phi_{n,\e}) \mathbbm{1}_{B_n} \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right]
	\\
	& \leq \bbE_{P^{n}_0}  \phi_{n,\e} 
	+ \bbE_{P^{n}_0} \left[ \mathbbm{1}_{B_n^C}  \right] 
	+ \bbE_{P^{n}_0} \left[ (1 - \phi_{n,\e}) \mathbbm{1}_{B_n} \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right],
	\label{eq:f3}
\end{align} 
where in the second inequality, we first divide the second term over set $B_n$ and its complement, and then use the fact that $  \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \leq 1$. The third inequality is due the fact that $\phi_{n,\e} \in[0,1]$.
Next, using Assumption~\ref{assump:Asf3} and~\ref{assump:Asf15} observe that on set $B_n$ 
\begin{align*}
	\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)  & \geq W^{\gamma} \int_{\Theta}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)
	\\
	& \geq W^{\gamma} e^{-(1+ C_2 +C_3 )n\e_n^2} \geq W^{\gamma} e^{-(1+ C_2 +C_3 )n\e^2}.
\end{align*}
Substituting  the equation above in the third term of equation~\eqref{eq:f3}, we obtain
\begin{align}
	\nonumber
	&	\bbE_{P^{n}_0} \left[  (1  - \phi_{n,\e}) \mathbbm{1}_{B_n}  \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] 
	\\
	\nonumber
	& \leq  W^{-{\gamma}} e^{(1+C_2 + C_3 )n\e^2} \bbE_{P^{n}_0} \left[ (1 - \phi_{n,\e}) \mathbbm{1}_{B_n} {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right]
	\\
	& \leq  W^{-{\gamma}} e^{(1+C_2 + C_3 )n\e^2} \bbE_{P^{n}_0} \left[ (1 - \phi_{n,\e}) {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right].
	\tag{$\star$}
\end{align} 
Now using Fubini's theorem observe that,
\begin{align*}
	(\star) & =  W^{-{\gamma}} e^{(1+C_2 + C_3 )n\e^2} {\int_{K_n} e^{\gamma R(a',\theta)}  \bbE_{P_\theta^n} \left[ (1 - \phi_{n,\e})  \right] d\Pi(\theta) } 
	\\
	\nonumber
	& \leq W^{-{\gamma}} e^{(1+C_2 + C_3 + C_4({\gamma}))n\e^2} \bigg[ {\int_{K_n \cap \{e^{\gamma R(a',\theta)} \leq e^{C_4({\gamma}) n\e^2} \} }  \bbE_{P_\theta^n} \left[ (1 - \phi_{n,\e})  \right] d\Pi(\theta) }
	\\
	\nonumber
	& \quad \quad \quad \quad \quad \quad \quad \quad + e^{-C_4({\gamma}) n\e^2} {\int_{K_n \cap \{e^{\gamma R(a',\theta)} > e^{C_4({\gamma}) n\e^2} \} } e^{\gamma R(a',\theta)}   d\Pi(\theta) } \bigg],
\end{align*}
where in the last inequality, we first divide the integral over set $\{\theta \in \Theta : e^{\gamma R(a',\theta)} \leq e^{C_4({\gamma})n\e^2} \}$ and its complement and then use the upper bound on $e^{\gamma R(a',\theta)}$ in the first integral. 
Now, it follows that 
\begin{align*}
	(\star) & \leq W^{-\gamma} e^{(1+C_2 + C_3 + C_4({\gamma}) )n\e^2} \left[ {\int_{K_n }  \bbE_{P_\theta^n} \left[ (1 - \phi_{n,\e})  \right] d\Pi(\theta) }  + e^{-C_4({\gamma}) n\e^2} {\int_{\{e^{\gamma R(a',\theta)} > e^{C_4({\gamma}) n\e^2} \} } e^{\gamma R(a',\theta)} d\Pi(\theta) } \right]
	\\
	&= W^{-\gamma} e^{(1+C_2 + C_3 + C_4({\gamma}) )n\e^2} \bigg[ {\int_{K_n \cap \Theta_n(\e) }  \bbE_{P_\theta^n} \left[ (1 - \phi_{n,\e})  \right] d\Pi(\theta) } + {\int_{K_n \cap \Theta_n(\e)^c }  \bbE_{P_\theta^n} \left[ (1 - \phi_{n,\e})  \right] d\Pi(\theta) } 
	\\ & \quad \quad \quad \quad \quad \quad \quad \quad +  e^{-C_4({\gamma}) n\e^2} {\int_{\{e^{\gamma R(a',\theta)} > e^{C_4({\gamma}) n\e^2} \} } e^{\gamma R(a',\theta)} d\Pi(\theta) } \bigg]
	\\
	& \leq W^{-\gamma} e^{(1+C_2 + C_3 + C_4({\gamma}) )n\e^2} \bigg[ {\int_{K_n \cap \Theta_n(\e) }  \bbE_{P_\theta^n} \left[ (1 - \phi_{n,\e})  \right] d\Pi(\theta) } + \Pi(\Theta_n(\e)^c) 
	\\ & \quad \quad \quad \quad \quad \quad \quad \quad +  e^{-C_4(\gamma)n\e^2} {\int_{\{e^{\gamma R(a',\theta)} > e^{C_4(\gamma)n\e^2} \} } e^{\gamma R(a',\theta)} d\Pi(\theta) } \bigg],
\end{align*}
where the second equality is obtained by  dividing  the first integral on set $\Theta_n(\e)$  and its complement, and the third inequality is due the fact that $\phi_{n,\e} \in[0,1]$. %and $\{e^{\gamma R(a',\theta)} > e^{C_4(\gamma)n\e_n^2} \} \subseteq \{e^{\gamma R(a',\theta)} > {C_4(\gamma)n\e_n^2} \}$. 
Now, using the equation above and Assumption~\ref{assump:Asf1},~\ref{assump:Asf2}, and~\ref{assump:Asf14} observe that 
\begin{align*}
	\bbE_{P^{n}_0} \left[  (1  - \phi_{n,\e}) \mathbbm{1}_{B_n}  \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] 
	&\leq W^{-\gamma} e^{(1+C_2 + C_3 + C_4(\gamma))n\e^2} \left[2 e^{-Cn \e^2} + e^{-(C_5(\gamma)+C_4(\gamma))n \e^2} \right].
\end{align*}
Hence, choosing $C,C_2,C_3, C_4(\gamma)$ and $C_5(\gamma)$ such that $ - 1 >  1 + C_2 + C_3 +C_4(\gamma) - \min(C,(C_4(\gamma) + C_5(\gamma)))$ implies

\begin{align}
	\bbE_{P^{n}_0} \left[  (1  - \phi_{n,\e}) \mathbb{I}_{B_n}  \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] \leq 3 W^{-\gamma} e^{-n\e^2}. \label{eq:eqf4}
\end{align}
By Assumption~\ref{assump:Asf1}, we have
\vspace{0em}
\begin{align}
	\bbE_{P^{n}_0}  \phi_{n,\e} & \leq C_0e^{-C n \e^2}. \label{eq:eq_1b} 
\end{align}
Therefore, substituting equation~\eqref{eq:eq_bn}, equation~\eqref{eq:eqf4}, and~\eqref{eq:eq_1b} into~\eqref{eq:f3}, we obtain
%\leq e^{-Cn \e_n^2} + e^{-\lambda n \e_n^2} + 2 e^{-n\e_n^2}
\begin{align}
	\bbE_{P^{n}_0} \left[  \frac {\int_{K_n} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right]  \leq (1+C_0+ 3W^{-\gamma}) e^{-C_{10} C_1 n \e^2}, \label{eq:eqf5}
\end{align}
where $C_{10} = \min \{\lambda,C, 1\}/ C_1$.
%Now using Lemma 6.4 of \cite{} , for some $\beta \leq C_{10}/2$. 
Using Fubini's theorem, observe that the LHS in the equation~\eqref{eq:eqf5} can be expressed as $\mu(K_n)$, where 
$$d\mu(\theta) = \bbE_{P^{n}_0} \left[\frac {   \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } \right] \Pi(\theta) e^{\gamma R(a',\theta)} d\theta.$$
Next, recall that the set $K_n = \{ \theta \in \Theta: L_n(\theta,\theta_0) > C_1n\e^2  \}$. Applying Lemma~\ref{lem:lem6.4} above with $X=L_n(\theta,\theta_0)$, $c_1 = (1+C_0+ 3W^{-\gamma})$ , $c_2= C_{10}$ , $t_0 = C_1 n \e_n^2$,  and for $0< \zeta \leq C_{10}/2 $, we obtain
\begin{align}
	\bbE_{P^{n}_0} \left[ \int_{\Theta}  e^{\zeta L_n  (\theta,\theta_0)} \frac {e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \Pi(\theta)} {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  d\theta \right]	\leq e^{\zeta C_{1}n \e_n^2} + (1+C_0+ 3W^{-\gamma}). 
	%\label{eq:eqf6}
\end{align}

\end{proof}
Further, we have another technical lemma, that will be crucial in proving the subsequent lemma that upper bounds the last term in the equation~\eqref{eq:eqf2}.
\begin{lemma}\label{lem:lem6.5}
	Suppose a positive random variable X satisfies
	\vspace{0em}
	$$\mathbb{P}(X\geq e^t) \leq c_1 \exp(-(c_2+1) t),$$
	for all $t \geq t_0>0$, $c_1>0 $, and $c_2>0$. Then,
	\vspace{0em}
	$$ \bbE[ X] \leq \exp(t_0) + \frac{c_1}{c_2}.$$
\end{lemma}
\begin{proof}
For any $Z_0 > 1$,
\vspace{0em}
\begin{align*}
	\bbE[ X] \leq Z_0 + \int_{Z_0}^{\infty} \mathbb{P} (X \geq  x) dx = Z_0+ \int_{\ln Z_0}^{\infty} \mathbb{P} (X \geq  e^y) e^y dy  \leq Z_0 + c_1 \int_{\ln Z_0}^{\infty} \exp(-c_2y) dy.
\end{align*}
Therefore, choosing $Z_0 = \exp(t_0)$,
\vspace{0em}
\begin{align*}
	\bbE[ X] \leq \exp(t_0) + \frac{c_1}{c_2} \exp(-c_2 t_0) \leq \exp(t_0) + \frac{c_1}{c_2}.
\end{align*}

\end{proof}
Next, we establish the following bound on the last term in equation~\eqref{eq:eqf2}.
\begin{lemma}
	Under Assumptions~\ref{assump:Asf1},~\ref{assump:Asf2},~\ref{assump:Asf3},~\ref{assump:Asf14},~\ref{assump:Asf15},  and for $ C_4(\gamma)+ C_5(\gamma) > C_2 + C_3 + 2$,
	\begin{align}
		\bbE_{P^{n}_0} \left[ \int_{\Theta}  \frac { e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)} {\int_{\Theta} \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }   \right]	\leq e^{C_{4}(\gamma)n \e_n^2} + 2C_4(\gamma).
		\label{eq:eqf12}
	\end{align}
	%where $C_{11}(\gamma) = \min \{\lambda,1+C_4(\gamma)\}/ C_4(\gamma)-1$ for any $\lambda>0$.
\end{lemma}
\begin{proof}
Define the  set 
\begin{align}
	M_n &: = \{ \theta \in \Theta : e^{\gamma R(a',\theta)} > e^{C_4(\gamma) n\e^2}  \}. %\quad \forall k \in \mathbb{N}, \\
\end{align}
Using the set $B_n$ in equation~\eqref{def:def1}, observe that the measure of the set $M_n$, under the posterior distribution satisfies, 
%to get a bound \textcolor{red}{on the first term of the RHS in equation~\eqref{eq:eqf2}}. Consider
\begin{align}
	\bbE_{P^{n}_0} \left[  \frac {\int_{M_n} \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] & \leq \bbE_{P^{n}_0} \left[ \mathbbm{1}_{B_n^c} \right]
	+ \bbE_{P^{n}_0} \left[ \mathbbm{1}_{B_n} \frac {\int_{M_n}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right].
	\label{eq:f9}
\end{align}
Now, the second term of equation~\eqref{eq:f9} can be  bounded as follows: recall Assumption~\ref{assump:Asf3} and the definition of set $B_n$, both together imply that,
\begin{align*}
	\bbE_{P^{n}_0} \left[  \mathbbm{1}_{B_n}  \frac {\int_{M_n}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta}   \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] & \leq  e^{(1+C_2 + C_3 )n\e^2} \bbE_{P^{n}_0} \left[  \mathbbm{1}_{B_n} {\int_{M_n} \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right]
	\\
	& \leq e^{(1+C_2 + C_3 )n\e^2} \bbE_{P^{n}_0} \left[  {\int_{M_n}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right].
	\tag{$\star \star$}
\end{align*}
Then, using Fubini's Theorem $(\star \star ) =   e^{(1+C_2 + C_3 )n\e^2} \Pi(M_n)$. Next, using the definition of set $M_n$ and  then Assumption~\ref{assump:Asf14}, we obtain
\begin{align*}
	\bbE_{P^{n}_0} \left[  \mathbbm{1}_{B_n}  \frac {\int_{M_n}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta}   \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] & \leq e^{(1+C_2 + C_3 )n\e^2} e^{-C_4(\gamma)n\e^2} \int_{M_n} e^{\gamma R(a',\theta)}d\Pi(\theta)
	%\\
    %&\leq e^{(1+C_2 + C_3 )n\e_n^2} e^{-C_4(\gamma)n\e_n^2} \int_{M'_n} e^{\gamma R(a',\theta)}d\Pi(\theta)
    \\
	& \leq e^{(1+C_2 + C_3 )n\e^2} e^{-C_4(\gamma)n\e^2} e^{-C_5(\gamma)n\e^2},
	%\\
	%& \leq e^{(1+C_2 + C_3 )n\e_n^2} e^{-C_4(\gamma)n\e_n^2} e^{-C_5(\gamma) n\e_n^2}
\end{align*}
%where the second inequality follows since $M_n\subseteq M_n':= \{ \theta \in \Theta : e^{\gamma R(a',\theta)} > {C_4(\gamma) n\e_n^2}  \}$ .
Hence, choosing the constants $C_2,C_3, C_4(\gamma)$ and $C_5(\gamma)$ such that  $ - 1 >  1 + C_2 + C_3  - C_5(\gamma)$ implies
\begin{align}
	\bbE_{P^{n}_0} \left[ \mathbbm{1}_{B_n}  \frac {\int_{M_n}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right] \leq e^{-(1+C_4(\gamma))n\e^2} \label{eq:eqf10}
\end{align}
Therefore, substituting~\eqref{eq:eq_bn} and~\eqref{eq:eqf10} into~\eqref{eq:f9}
%\leq e^{-Cn \e_n^2} + e^{-\lambda n \e_n^2} + 2 e^{-n\e_n^2}
\begin{align}
	\bbE_{P^{n}_0} \left[  \frac {\int_{M_n}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }  \right]  \leq 2 e^{-C_4(\gamma) (C_{11}(\gamma)+1)n \e^2}, \label{eq:eqf11}
\end{align}
where $C_{11} = \min \{\lambda,1+C_4(\gamma)\}/ C_4(\gamma)-1$.
%Now using Lemma 6.4 of \cite{} , for some $\beta \leq C_{11}(\gamma)/2$ and using the fact that $e^x>x~\forall x>0$.
Using Fubini's theorem, observe that the RHS in~\eqref{eq:eqf11} can be expressed as $\nu(M_n)$, where the measure $$d\nu(\theta) = \bbE_{P^{n}_0} \left[\frac {   \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  } {\int_{\Theta}   \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } \right] d \Pi(\theta).$$ 
Applying Lemma~\ref{lem:lem6.5} for $X=e^{\gamma R(a',\theta)}$,$c_1 = 2$ , $c_2= C_{11}(\gamma)$ , $t_0 = C_4(\gamma) n \e_n^2$ and $\lambda\geq 1+C_4(\gamma)$, we obtain
\begin{align}
	\bbE_{P^{n}_0} \left[ \int_{\Theta}  \frac { e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)} {\int_{\Theta} \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }   \right]	\leq e^{C_{4}n \e_n^2} + \frac{2}{C_{11}(\gamma)} \leq e^{C_{4}n \e_n^2} + 2C_4(\gamma) .
	%\label{eq:eqf12}
\end{align}

\end{proof}

\begin{proof}{Proof of Theorem~\ref{thrm:thm1}:}
Finally, recall~\eqref{eq:eqf2},
\begin{align}
	\nonumber
	\zeta \bbE_{P^{n}_0}& \left[ \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right]  
	\\ 
	\nonumber
	\leq & \log  \bbE_{P^{n}_0} \left[ \int_{\Theta}  e^{\zeta L_n  (\theta,\theta_0)} \frac {e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) } {\int_{\Theta} e^{\gamma R(a',\theta)}  \ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta) }   \right] +  \inf_{Q \in \sQ} \bbE_{P^{n}_0} \bigg[  \scKL(Q(\theta)\|\Pi(\theta|\nX)) 
	\\
	& - \gamma \inf_{a \in  \mathcal{A}} \bbE_Q[R(a,\theta)] \bigg] +\log  \bbE_{P^{n}_0} \left[ \int_{\Theta} e^{\gamma R(a',\theta)}  \ \frac{\prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)}{\int_{\Theta} \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\Pi(\theta)}  \right] . 
\end{align}
Substituting~\eqref{eq:eqf12} and ~\eqref{eq:eqf6} into the above equation and then using the  definition of $\eta_n^R(\gamma)$, we get
\begin{align}
	\nonumber
	\bbE_{P^{n}_0}& \left[ \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right]  \\
	\nonumber
	& \leq \frac{1}{\zeta} \left\{ \log(e^{\zeta C_{1}n \e_n^2} + (1+C_0+ 3W^{-\gamma}))  + \log \left( e^{C_{4}(\gamma) n \e_n^2} + 2C_4(\gamma) \right)  + n \eta_n^R(\gamma)  \right\}
	\\
	%\nonumber
	%& \leq (C_{1} + \frac{\omega}{\beta} C_4(\gamma) )n \e_n^2 + \frac{1}{\beta}n \eta_n^R^2(a) + \frac{(1+C_0+ 3W^{-\gamma})e^{(-\beta C_{1}n \e_n^2)}  }{\beta} 
	%\\
	\nonumber
	& \leq \left( C_{1}+ \frac{1}{\zeta} C_4(\gamma) \right) n \e_n^2  + \frac{1}{\zeta}n \eta_n^R(\gamma)  +\frac{(1+C_0+ 3W^{-\gamma})e^{(-\zeta C_{1}n \e_n^2)}   }{\zeta}  + \frac{2C_4(\gamma)e^{ - C_{4}(\gamma)n \e_n^2}}{\zeta},
\end{align}
where the last inequality uses the fact that $\log x \leq x -1$. Choosing $ \zeta= C_{10}/2= \frac{\min(C,\lambda,1)}{2C_1}$, 
%and $\omega= C_{11}(\gamma)/2 = \frac{\min(\lambda,1)}{2C_4(\gamma)}$, we get 
\begin{align}
	\nonumber
	\bbE_{P^{n}_0}& \left[ \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right]  \\
	& \leq M(\gamma) n (\e_n^2)  + M' n \eta_n^R(\gamma)  +\frac{2 (1+C_0+ 3W^{-\gamma})e^{(- \frac{C_{10}}{2}n \e_n^2)}  }{C_{10}} + \frac{4C_{4}(\gamma) e^{ - C_{4}(\gamma)n \e_n^2}}{C_{10}}  \label{eq:lc2}
	%\frac{4 + 4(1+(C_4(\gamma))^{-1})e^{ - \frac{C_11}{2} C_{4}n \e_n^2}}{C_{10}C_{11}(\gamma)},
\end{align}
where $M(\gamma)= C_{1}+ \frac{1}{\zeta} C_4(\gamma)$ and $M'=\frac{1}{\zeta}$ depend on $C,C_1, C_4(\gamma) ,W\text{ and } \lambda$. Since the last two terms in~\eqref{eq:lc2} decrease and the first term increases as $n$ increases, we can choose $M'$ large enough, %$\tilde{n}(C_0,C_4(\gamma),C_{10},C_{11}(\gamma),M,a)$, 
such that for all $n \geq 1$
%\[M' n (\e_n^2  + \eta_n^R^2(a) ) > \frac{2 (1+C_0+ 3W^{-\gamma})e^{(- \frac{C_{10}}{2}n \e_n^2)}  }{C_{10}} + \frac{4e^{ - C_{4}n \e_n^2}}{C_{11}(\gamma)C_{10}}, \]
\[ M' n \eta_n^R(\gamma)  > \frac{2 (1+C_0+ 3W^{-\gamma})  }{C_{10}} + \frac{4C_{4}(\gamma)}{C_{10}}, \]
and therefore for $M=2M'$,
\begin{align}
	\bbE_{P^{n}_0} \left[ \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right] \leq M(\gamma) n (\e_n^2)  + M n \eta_n^R(\gamma). \label{eq:lc3}
	%\frac{4 + 4(1+(C_4(\gamma))^{-1})e^{ - \frac{C_11}{2} C_{4}n \e_n^2}}{C_{10}C_{11}(\gamma)},
\end{align}

Also, observe that  the LHS in  the above equation is always  positive, therefore $M(\gamma)  \e_n^2  + M  \eta_n^R(\gamma)\geq 0 \ \forall n \geq 1$ and $\gamma>0$.

\end{proof}



%%%%%%%%%%%%%%%%%

%\subsection{Proof of Theorem~\ref{thrm:thm1a}.}
%\begin{proof}{Proof of lemma~\ref{thm:thm1}:}
%Refer Theorem 2.1 of \cite{Zhang2018}.
%\end{proof}

\subsection{Proof of Theorem~\ref{thrm:OGValue} and~\ref{thrm:OGdecision} }

\begin{lemma}~\label{lem:Lemma3}
    Given $a' \in \mathcal{A}$ and for a constant M, as defined in Theorem~\ref{thrm:thm1} 
    \begin{align}
        \bbE_{P^{n}_0} \left[ \sup_{a \in \mathcal{A}} \left \vert \bbE_{\qrs}[R(a,\theta)] - R(a,\theta_0) \right \vert \right]  \leq  \left [M (\e_n^2 + \eta_n^{R}(\gamma))\right ]^{\frac{1}{2}}.
    \end{align}
\end{lemma}



\begin{proof}
    First, observe that
    \begin{align*}
        \left( \sup_{a \in \mathcal{A}} \left\vert \bbE_{\qrs}[R(a,\theta)] - R(a,\theta) \right\vert \right)^2 & \leq 
        \left( \int \sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta_0)\vert  d\qrs \right)^2
        \\
        &	\leq \int \left(\sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta_0) \vert \right)^2 d\qrs,
    \end{align*}
    where the last inequality follows from Jensen's inequality. Now, using the Jensen's inequality again 
    \begin{align*}
        & \left ( \bbE_{P^{n}_0} \left[ \sup_{a \in \mathcal{A}} \left\vert \bbE_{\qrs}[R(a,\theta)] - R(a,\theta_0) \right\vert \right] \right)^2 
        \\ 
        & \quad \quad \leq  \bbE_{P^{n}_0} \left[  \left( \sup_{a \in \mathcal{A}} \left\vert \bbE_{\qrs}[R(a,\theta)] - R(a,\theta_0) \right\vert \right)^2 \right].
    \end{align*}
    Now, using Theorem~\ref{thrm:thm1} the result follows immediately.
    
\end{proof}
\begin{proof}[Proof of Theorem~\ref{thrm:OGValue}]
    %Let $R(a,\theta)= f(G(a,\theta))$, where $f:\bbR\to \bbR$
    %is a monotonic function. Now 
    Observe that 
    \begin{align}
        \nonumber
        %\Psi&\left( d_h(\ars, \underset{a \in \mathcal{A} }{\arg \min}   ~ f(G(a,\theta_0)) ) \right) 
        %\\
        %\nonumber
        %&\leq 
        &R( \ars,\theta_0) - \inf_{z \in \mathcal{A}} R(z,\theta_0)
        \\
        \nonumber
        & = \vert  R( \ars,\theta_0) - \inf_{z \in \mathcal{A}} R(z,\theta_0)  \vert 
        \\
        \nonumber
        & =  R( \ars,\theta_0) - \int   R(\ars,\theta)  dQ^*_{\ars,\gamma}(\theta|\nX)   +   \int   R(\ars,\theta)  dQ^*_{\ars,\gamma}(\theta|\nX)  - \inf_{z \in \mathcal{A}} R(z,\theta_0) 
        \\
        \nonumber
        & \leq  \left \vert  R( \ars,\theta_0) - \int   R(\ars,\theta)  dQ^*_{\ars,\gamma}(\theta|\nX)   \right \vert + \left \vert  \int   R(\ars,\theta)  dQ^*_{\ars,\gamma}(\theta|\nX)  - \inf_{a \in \mathcal{A}} R(a,\theta_0)  \right \vert 
        \\
        \nonumber
        & \leq 2 \sup_{a \in \mathcal{A}} \left\vert \int  R(a,\theta) dQ^*_{\ars,\gamma}(\theta|\nX) - R(a,\theta_0) \right\vert. 
        \label{eq:eqt21}
    \end{align}
    
    Given $\ars \in \mathcal{A}$ and for a constant M (defined in Theorem~\ref{thrm:thm1}), we have from Lemma~\ref{lem:Lemma3} for $a'=\ars$
    \begin{align}
        \bbE_{P^{n}_0} \left[ \sup_{a \in \mathcal{A}} \left \vert \int  R(a,\theta) dQ^*_{\ars,\gamma}(\theta|\nX) - R(a,\theta_0) \right \vert \right]  \leq  \left [M (\e_n^2 + \eta_n^{R}( \gamma))\right ]^{\frac{1}{2}}.
    \end{align}
    
    It follows from above that the $P_0^n-$ probability of the following event is at least $ 1- \tau^{-1}$:
    \begin{align}
        \bigg\{ \nX:   R( \ars,\theta_0) - \inf_{z \in \mathcal{A}} R(z,\theta_0)  \leq 2\tau  \left[ M (\e_n^2 + \eta_n^R(\gamma)) \right]^{\frac{1}{2}}  \bigg\}.
    \end{align}
\end{proof}





\begin{proof}[Proof of Theorem~\ref{thrm:OGdecision}:]
    Since, the above result holds for any $a' \in \sA$, fix $a' =\ars $ and observe  that for any $\gamma>0$ and $\tau>0$, the result in Lemma~\ref{lem:Lemma3} implies that $P_0^n-$ probability of 
    \begin{align}
        \left\{ \left[ M (\e_n^2 + \eta_n^R(\gamma)) \right]^{-\frac{1}{2}} \sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta) dQ^*_{\ars,\gamma}(\theta|\nX) -R(a,\theta_0) \right\vert > \tau \right\}
    \end{align}
    %\in \underset{z \in \mathcal{A} }{\arg \min} \int   G(z,\theta) q^*(\theta| \nX) d\theta  $
    is at most $\tau^{-1}$. For $\ars$, it follows from the definition of $ \Psi(\cdot)$ that
    \begin{align}
        \nonumber
        \Psi&\left( d_h(\ars, \underset{a \in \mathcal{A} }{\arg \min}   ~ R(a,\theta_0) ) \right) 
        \\
        \nonumber
        &\leq R(\ars,\theta_0) - \inf_{z \in \mathcal{A}} R(a,\theta_0) 
        \\
        \nonumber
        %& = \vert  G( \ars,\theta_0) - \inf_{z \in \mathcal{A}} G(z,\theta_0)  \vert 
        %\\
        & =  R(\ars,\theta_0) - \int   R(\ars,\theta) dQ^*_{\ars,\gamma}(\theta|\nX)   +   \int   R(\ars,\theta) dQ^*_{\ars,\gamma}(\theta|\nX)  - \inf_{z \in \mathcal{A}} R(z,\theta_0)
        \\
        \nonumber
        & \leq  \left \vert  R(\ars,\theta_0) - \int   R(\ars,\theta) dQ^*_{\ars,\gamma}(\theta|\nX)   \right \vert + \left \vert  \int   R(\ars,\theta) dQ^*_{\ars,\gamma}(\theta|\nX)  - \inf_{a \in \mathcal{A}} R(a,\theta_0)  \right \vert 
        \\
        & \leq 2 \sup_{a \in \mathcal{A}} \left\vert \int  R(a,\theta) dQ^*_{\ars,\gamma}(\theta|\nX) - R(a,\theta_0) \right\vert. 
        \label{eq:eqt21}
    \end{align}
    It follows from the above inequality that
    \begin{align}
        \nonumber
        \bigg\{ \left[ M (\e_n^2 + \eta_n^R(\gamma)) \right]^{-\frac{1}{2}} \Psi\bigg( &d_h(\ars, \underset{z \in \mathcal{A} }{\arg \min}   ~ R(a,\theta_0) ) \bigg) > 2 \tau \bigg\}
        \\
        & \subseteq \left\{ \left[ M (\e_n^2 + \eta_n^R(\gamma)) \right]^{-\frac{1}{2}} \sup_{a \in \mathcal{A}} \left\vert \int  R(a,\theta) dQ^*_{\ars,\gamma}(\theta|\nX) - R(a,\theta_0) \right\vert > \tau \right\} .
        \label{eq:eq32}
    \end{align} 
    Therefore, using the condition on the growth function in the statement of the theorem that, $\frac{ \Psi\left(d_h\left(\ars, \underset{a \in \mathcal{A} }{\arg \min}   ~ R(a,\theta_0) \right)\right)}{d_h\left(\ars, \underset{a \in \mathcal{A} }{\arg \min}   ~ R(a,\theta_0) \right)^{\delta}} =  \kappa,$ the $P_0^n-$ probability of the following event is at least $ 1- \tau^{-1}$:
    \begin{align}
        \bigg\{    d_h(\ars, \underset{a \in \mathcal{A} }{\arg \min}   ~ R(a,\theta_0) )  \leq \tau^{\frac{1}{\delta}} \left[ \frac{2 \left[ M (\e_n^2 + \eta_n^R(\gamma)) \right]^{\frac{1}{2}} }{ \kappa } \right]^{\frac{1}{\delta}} \bigg\}.
    \end{align}
    %Using the monotonicity of the function $f(\cdot)$, it follows that $\underset{a \in \mathcal{A} }{\arg \min}  ~ R(a,\theta_0) = \underset{a \in \mathcal{A} }{\arg \min}  ~ G(a,\theta_0) $ and hence 
    This concludes the proof.
    
   
\end{proof}

%\begin{proof}{Proof of Theorem~\ref{prop:prop2}(2):} The proof follows similar steps till equation~\eqref{eq:eq32} in the proof above and then uses the condition on the growth function $\Psi^f(\cdot)$ given in the statement of the theorem for all $n\geq n_0$.    
%\end{proof}



%\begin{proof}{Proof of Corollary~\ref{corr:cor5}:}
%    Using triangular inequality it is straightforward to see that
%    \begin{align*}
%        & P^{n}_0\left( d_h(\aos, \ars)     > 2\left[\frac{2 \tau \left[ M_n \e_n^2 \right]^ { \frac{1}{2} }}{C^1} \right]^\frac{1}{\delta} + 2\left[\frac{2 \tau \left[ M_n (\e_n^2 + \eta_n^R(\gamma)) \right]^{\frac{1}{2}}}{C^f} \right]^\frac{1}{\delta} \right)
%        \\
%        &\leq P^{n}_0\left( d_h(\aos, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) ) + d_h(\ars, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) )     > 2\left[\frac{2 \tau \left[ M_n \e_n^2 \right]^ { \frac{1}{2} }}{C^1} \right]^\frac{1}{\delta} +2 \left[\frac{2 \tau \left[ M_n (\e_n^2 + \eta_n^{R}(\gamma)) \right]^{\frac{1}{2}}}{C^f} \right]^\frac{1}{\delta} \right)
%        \\
%        &\leq P^{n}_0\left( d_h(\aos, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) )     > \left[\frac{2 \tau \left[ M_n \e_n^2 \right]^ { \frac{1}{2} }}{C^1} \right]^\frac{1}{\delta} + \left[\frac{2 \tau \left[ M_n (\e_n^2 + \eta_n^{R}(\gamma)) \right]^{\frac{1}{2}} }{C^f} \right]^\frac{1}{\delta} \right)
%        \\
%        & \quad+
%        P^{n}_0\left(  d_h(\ars, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) )     > \left[\frac{2 \tau \left[ M_n \e_n^2 \right]^ { \frac{1}{2} }}{C^1} \right]^\frac{1}{\delta} + \left[\frac{2 \tau \left[ M_n (\e_n^2 + \eta_n^{R}(\gamma)) \right]^{\frac{1}{2}} }{C^f} \right]^\frac{1}{\delta} \right)
%        \\
%        & \leq P^{n}_0\left( d_h(\aos, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) )     > \left[\frac{2 \tau \left[ M_n \e_n^2 \right]^ { \frac{1}{2} }}{C^1} \right]^\frac{1}{\delta}  \right) +
%        P^{n}_0\left(  d_h(\ars, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) )     >  \left[\frac{2 \tau \left[ M_n (\e_n^2 + \eta_n^{R}(\gamma)) \right]^{\frac{1}{2}} }{C^f} \right]^\frac{1}{\delta} \right).
%    \end{align*}
%    
%    The proof follows immediately using Theorem~\ref{prop:prop2} and Corollary  \ref{corr:cor4}.%~\eqref{eq:os}. 
%    
%\end{proof}

%\subsection{Proof of Proposition~\ref{prop:prop3}}

%\subsection{Proof of Theorem~\ref{thm:thm3}:}
%
%\begin{proof}{Proof of Lemma~\ref{lem:cover2}:}
%%		Let $\theta \in [\theta_0 - k\e, \theta_0 + k\e ]^s \subset \mathbb R^s$. Now consider a set $H_i= \{\theta_i^0,\theta_i^1, \ldots \theta_i^M, \theta_i^{M+1} \}$ and $H=\bigotimes_s H_i $ with $M= \lfloor\frac{2 k\e}{\delta'}\rfloor$, where  $\theta^j_i = \theta_0 - k\e + i\delta'$ for $j=\{0,1,\dots , M \}$ and $\theta_i^{M+1}= \theta_0 + k\e$. Observe that for any $\theta \in [\theta_0 - k\e, \theta_0 + k\e ]^s$, there exists a $\theta^j \in  H$ such that $\| \theta - \theta^j \| < \delta'$. Hence union of the $\delta'-$balls for each element in set $H$ covers $[\theta_0 - k\e, \theta_0 + k\e ]^s$, therefore $N(\delta',[\theta_0 - k\e, \theta_0 + k\e ]^s, \|\cdot\|) = (M+2)^s$.	
%Since, $G(a,\theta)$ is locally Lipschitz in $\theta$ due to Assumption~\ref{assump:Asf4} and logarithmic function is also locally Lipschitz for a given $a$, therefore the result follows immediately using similar arguments as in Lemma~\ref{lem:cover}.
%
%
%%	for any $\theta \in [\theta_0 - k\e, \theta_0 + k\e ]^s$
%%	\begin{align}
%%	 \sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta^j) \vert \leq \sup_{a \in \mathcal{A}} \frac{1}{\underset{\theta \in [\theta_0 - k\e, \theta_0 + k\e ] }{\min} G(a,\theta) } \vert G(a,\theta) - G(a,\theta^j) \vert \leq C \| \theta - \theta^j \| \leq C \delta',
%%	\end{align}
%%	where $C = \sup_{a \in \mathcal{A}} \frac{K(a)}{\underset{\theta \in [\theta_0 - K\e, \theta_0 + K\e ] }{\min} G(a,\theta) }$. Hence $\delta'$-cover of set $[\theta_0 - k\e, \theta_0 + k\e ]^s$ is $C\delta'$ cover of set $T_2(\e)$ with $k= 1/C$.
%%	
%%		Finally,
%%	\begin{align}
%%	N(C \delta', T(\e), d ) \leq (M+2)^s \leq \left( \frac{2 k\e}{\delta'} + 2 \right)^s=   \left( \frac{2 \e}{C\delta'} + 2 \right)^s
%%	\end{align}
%%	
%%	which implies for $\delta = C\delta'$, 
%%	\begin{align}
%%	N(\delta, T(\e), d ) \leq  \left(\frac{2 \e}{\delta} + 2 \right)^s.  
%%	\end{align}
%
%%	Using continuity of logarithm function, for $\forall \delta> 0 \exists C \gamma(\delta)>0$ for some constant $C>0$ such that  
%%	\begin{align}
%%		\sup_{a \in \mathcal{A}}  \vert G(a,\theta) - G(a,\theta^j) \vert \leq C \gamma(\delta)  \implies d_2(\theta,\theta_j) < \delta.	
%%		\end{align} 
%%	
%%	Since logarithm is an increasing function, note that $\gamma(\delta)$ is also increasing in $\delta$. From Assumption~\ref{assump:Asf4} we know that 
%%	
%%	\begin{align}
%%	\vert \theta - \theta^j \vert \leq  \gamma(\delta) \implies	\sup_{a \in \mathcal{A}}  \vert G(a,\theta) - G(a,\theta^j) \vert \leq C \gamma(\delta) 
%%		\end{align} 
%%	
%%	 Hence $\delta$-cover of set $T_2(\e)$ is $C \gamma(\delta)  $  cover of $T(C\gamma(\e) )$. Therefor using Lemma~\ref{lem:cover2}  
%%	 
%%	\begin{align}
%%	N(\delta, T_2(\e), d ) =N(C \gamma(\delta), T(C\gamma(\e)), d ) \leq \frac{2 \gamma(\e)}{\gamma(\delta)} + 2
%%	\end{align}
%
%%	which implies 
%%	\begin{align}
%%	N(\delta, T(\e), d ) \leq \frac{2 \e}{\delta} + 2   
%%	\end{align}
%%	
%\end{proof}
%
%\begin{proof}{Proof of Lemma~\ref{lem:ass11}:}
%Recall $d_2(\theta,\theta_0)= \sup_{a \in  \mathcal{A}} |R(a,\theta)- R(a,\theta_0)|$ and $T_2(\e) = \{P_{\theta} : d_2(\theta,\theta_0)<\e \}$.
%Using Lemma~\ref{lem:cover2}, observe that for every $ \e > \e_n > 0$
%\begin{align}
%	N\left(\frac{\e}{2}, \{ \theta: \e \leq d_2(\theta,\theta_0) \leq 2\e \}, d_2 \right) \leq N\left(\frac{\e}{2}, \{ \theta: d_2(\theta,\theta_0) \leq 2\e \}, d_2 \right) \leq 10^s.
%\end{align}
%
%Using Assumption~\ref{assump:Asf16} and the fact that total variation distance is bounded above by Hellinger distance, we have
%\[d_2(\theta,\theta_0) \leq  \sup_{a \in  \mathcal{A}} \frac{K_1(a)}{W} d_{TV}(\theta,\theta_0) \leq \sup_{a \in  \mathcal{A}} \frac{K_1(a)}{W} h(\theta,\theta_0). \]
%It follows from above two observations and Lemma~\ref{lem:ggv71} that for every $\e > \e_n>0$ there exists sequence of tests $\{\phi_{n,\e}\}$ such that 
%\begin{align}
%	\bbE_{P^{n}_0}[ \phi_{n,\e} ]  &\leq 10^s  \frac{\exp(-C' n \e^2 )}{1-\exp(-C'n\e^2)},  \\
%	\underset{\{ \theta\in \Theta : d_2(\theta,\theta_0) \geq \epsilon  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_{n,\e} ] &\leq  \exp(-C' n \e^2 ),\label{eq:eq311}
%\end{align} 
%where $C' = \frac{W^2}{2 (\sup_{a\in \mathcal{A}} K_1(a))^2}$. Now, using using  similar arguments as for the set $T_2(\e)$ in the NVB case in Lemma~\ref{lem:ass1}, the result follows.
%
%\end{proof}
%
%\begin{proof}{Proof of Theorem~\ref{thm:thm3}:}
%Using Lemma~\ref{lem:ass11} observe that for any $\Theta_n(\e) \subseteq \Theta$,  $L_n(\theta,\theta_0)$ satisfies Assumption~\ref{assump:Asf1} with $C_0=2* 10^s$,$C = \frac{W^2 C_1}{2(\sup_{a\in \mathcal{A}} K_1(a))^2}$ and for any $C_1>1$, since 
%\begin{align*}
%	\underset{\{ \theta\in \Theta_n(\e) : L_n(\theta,\theta_0) \geq C_1 n \epsilon_n^2  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_{n,\e} ] \leq \underset{\{ \theta\in \Theta : L_n(\theta,\theta_0) \geq C_1 n \epsilon_n^2 \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_{n,\e} ] &\leq  \exp(-C n \e_n^2 ).
%\end{align*}
%Hence, applying Theorem~\ref{thm:thm2} for a fix $a_0 \in \sA$ and  using the definition of $\eta_n^{R}(1)(\gamma)$, the result follows.
%
%%for $L_n(\theta,\theta_0)$, as defined in \eqref{eq:loss},
%%\begin{align}
%%\bbE_{P^{n}_0} \left[ \int \left(\sup_{a \in \mathcal{A}} \vert G(a,\theta) - G(a,\theta_0) \vert \right)^2 q^*(\theta| \nX) d\theta \right] \leq M (\e_n^2 + \gamma_n^2), \label{eq:finB}
%%\end{align}
%%for some constant M,  where 
%%$$ \gamma_n^2 = \frac{1}{n} \inf_{Q \in \sQ} \bbE_{P^{n}_0} [\scKL({q}(\theta)\|\Pi(\theta|\nX)) ].  	$$
%
%\end{proof}
%
%
%
%%\begin{proof}{Proof of Theorem~\ref{corr:cor31}:}
%%	The result follows immediately from the following inequality 
%%	\begin{align*}
%%	\vert V_{q^*_{a_0}} - V_0 \vert \leq  \sup_{a \in \mathcal{A}} \left\vert  \int   R(a,\theta) q^*_{a_0}(\theta| \nX) d\theta - R(a,\theta_0) \right\vert .
%%	\end{align*}
%%	
%%\end{proof}
%
%
%
%








%\subsection{Proof of Proposition~\ref{prop:eta_n}}
\subsection{Proofs in Section~\ref{sbsec:PropEta}}
\begin{proof}[Proof of Proposition~\ref{prop:eta_n}]

Using the definition of  $\eta_n^R( \gamma)$ and the posterior distribution $\Pi(\theta|\nX)$, observe that
%,
\begin{align}
	\nonumber
	n\eta_n^R(\gamma) &= \inf_{Q \in \sQ} \bbE_{P^{n}_0} \left[  \scKL(Q(\theta)\|\Pi(\theta|\nX)) 
	- \gamma  \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] \right]
	\\
	\nonumber
	&= \inf_{Q \in \sQ} \bbE_{P^{n}_0} \left[  \scKL(Q(\theta)\|\Pi(\theta)) + \int_{\Theta}   	dQ(\theta)  \log \left( \frac{\int d\Pi(\theta)p(\nX|\theta) }{p(\nX|\theta)} \right) 
	- \gamma  \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] \right]
	\\
	\nonumber
	&= \inf_{Q \in \sQ} \left[ \scKL(Q(\theta)\|\Pi(\theta) ) - \gamma  \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] + \bbE_{P^{n}_0} \left[  \int_{\Theta}   	dQ(\theta)  \log \left( \frac{\int d\Pi(\theta)p(\nX|\theta) }{p(\nX|\theta)} \right) \right]\right] .
\end{align} 
Now, using  Fubini's in the last term of the equation above, we obtain
\begin{align}
	\nonumber
	n\eta_n^R(\gamma) &=  \inf_{Q \in \sQ} \Bigg[ \scKL(Q(\theta)\|\Pi(\theta) ) - \gamma  \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] 
	\\
	&\quad + \bbE_Q \left[ \scKL \left(dP^{n}_0\| p(\nX|\theta) \right) - \scKL\left( dP^{n}_0 \bigg\| \int d\Pi(\theta)p(\nX|\theta) \right)  \right]\Bigg] .
\end{align} 
Observe that, $\int_{\sX^n}\int d\Pi(\theta)p(\nX|\theta) d\nX = 1$. Since, \scKL \ is always non-negative, it follows from the equation above that
\begin{align}
	\nonumber
	&\eta_n^R(\gamma) 
	\\
	\nonumber
	&\leq \frac{1}{n} \inf_{Q \in \sQ} \left[ \scKL\left(Q(\theta)\|\Pi(\theta) \right) - \gamma  \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] + \bbE_Q \left[ \scKL\left(dP^{n}_0\| p(\nX|\theta) \right) \right]  \right]
	\\
	&\leq \frac{1}{n} \inf_{Q \in \sQ} \left[ \scKL\left(Q(\theta)\|\Pi(\theta) \right) + \bbE_Q \left[ \scKL\left(dP^{n}_0\| p(\nX|\theta) \right) \right]  \right] - \frac{1}{n} \gamma  \inf_{Q \in \sQ} \inf_{a \in \sA}  \bbE_Q[R(a,\theta)],
	\label{eq:eq1}
\end{align}
where the last inequality follows from the following fact, for any functions $f(\cdot)$ and
\vspace{0em} $g(\cdot)$, $$\inf (f -g) \leq \inf f - \inf g.$$
Recall $\e_n'\geq \frac{1}{\sqrt{n}}$. 
%such that
%\begin{align}
%	- \frac{1}{n} \gamma  \inf_{Q \in \sQ} \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] \leq \gamma C_8 \e_n'^2. 
%	\label{eq:eq1a}
%\end{align}
Now, using Assumption~\ref{assump:Asf11}, it is straightforward to observe that the first term in~\eqref{eq:eq1}, 
\begin{align}
	\frac{1}{n} \inf_{Q \in \sQ} \left[ \scKL\left(Q(\theta)\|\Pi(\theta) \right) + \bbE_Q \left[ \scKL\left(dP^{n}_0\| p(\nX|\theta) \right) \right]  \right] \leq C_9 \e_n'^2. 
	\label{eq:eq1b}
\end{align}
Now consider the last term in~\eqref{eq:eq1}. Notice that the coefficient of $\frac{1}{n}$ is independent of $n$ and is bounded from below. Therefore, there exist a constant $C_8=-  \inf_{Q \in \sQ} \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] $, 
such that with equation~\eqref{eq:eq1b} it follows  that $\eta_n^R(\gamma) \leq \gamma  n^{-1}C_8 +C_9\e_n'^2$ and the result follows.
%Since, $\inf_{Q \in \sQ} \left[ \scKL\left(Q(\theta)\|\Pi(\theta) \right) - \gamma  \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] \right] < \infty, \forall n \geq 1$ and $n\e_n^2 \geq 1$, therefore there exists a constant $C_8>0$ such that 
%\[\frac{1}{n}\left | \inf_{Q \in \sQ} \left[  \scKL\left(Q(\theta)\|\Pi(\theta) \right) - \gamma  \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] \right] \right| \leq C_8 \e_n^2. \]
%\textcolor{red}{the argument above is not complete}


\end{proof}

%\subsection{Proof of Proposition~\ref{prop:eta_gamma}}
\begin{proof}[{Proof of Proposition~\ref{prop:eta_gamma}}]
    
    First recall that
    \begin{align} 
        \nonumber
        n\eta_n^R(\gamma) &= \inf_{Q \in \sQ} \bbE_{P^{n}_0} \left[  \scKL(Q(\theta)\|\Pi(\theta|\nX)) 
        - \gamma \inf_{a \in  \mathcal{A}} \bbE_Q[R(a,\theta)] \right]
        \\
        &= \inf_{Q \in \sQ} \bbE_{P^{n}_0} \left[  \scKL(Q(\theta)\|\Pi(\theta|\nX))  \right]
        - \gamma \inf_{a \in  \mathcal{A}} \bbE_Q[R(a,\theta)]. 
        \label{eq:eqeta}
    \end{align}
    
    Observe that the optimization problem is equivalent to solving :
    %\begin{align} \max_{q \in \mathcal M} \left\{ \mathbb
    %    E_q[R(a,\theta)] - 
    %    \frac{1}{\gamma}\text{KL}(q||\pi_n) \right\}=-\frac{1}{\gamma}\min_{q \in \mathcal M} \left\{ 
    %    \text{KL}(q||\pi_n)- \gamma \mathbb
    %    E_q[R(a,\theta)]  \right\}
    %\end{align}
    %which is equivalent to solving:
    \begin{align} 
        \min_{Q \in \sQ} \bbE_{P^{n}_0} \left[  \scKL(Q(\theta)\|\Pi(\theta|\nX))  \right] \text{ s.t. } 
        - \inf_{a \in  \mathcal{A}} \bbE_Q[R(a,\theta)] \leq 0 .
    \end{align}
    
    %The above problem is primal feasible if
    %$-\mathbb
    %E_{q^*}[R(a,\theta)] \leq 0 $ and dual feasible when  $\gamma>0$.
    Now for any $\gamma>0$, $Q^*_{\gamma}(\theta) \in \sQ$ that minimizes the objective in~\eqref{eq:eqeta} is primal feasible if
    \[- \inf_{a \in  \mathcal{A}} \int_{\Theta}  dQ^*_{\gamma}(\theta) R(a,\theta)	  \leq 0. \]
    
    
    Therefore, it is straightforward to  observe that 
    as $\gamma$ increases $n\eta_n^R(\gamma)$ decreases that is
    \[ \bbE_{P^{n}_0} \left[  \int_{\Theta}   	dQ^*_{\gamma}(\theta)  \log \frac{dQ^*_{\gamma}(\theta)} { \Pi(\theta|\nX)  }   
    - \gamma \inf_{a \in  \mathcal{A}} \int_{\Theta}  dQ^*_{\gamma}(\theta) R(a,\theta)	  \right].\]
    
\end{proof} 

\begin{proof}{Proof of Corollary~\ref{corr:cor1a}:}
    For any $\delta>0$, using Markov inequality
    \begin{align*}
        P_0^n \left( Q_{a',\gamma}^* \left[ \left\{  \frac{1}{n}L_n(\theta,\theta_0) > M_n (\e_n^2 + \eta_n^R(\gamma))  \right\} \Big\vert \nX \right] > \delta \right) &\leq \frac{1}{\delta} \bbE_{P^{n}_0}  Q_{a',\gamma}^* \left[ \left\{  \frac{1}{n}L_n(\theta,\theta_0) > M_n (\e_n^2 + \eta_n^R(\gamma))  \right\} \Big\vert \nX \right] 
        \\
        &\leq \frac{1}{n \delta M_n (\e_n^2 + \eta_n^R(\gamma))} \bbE_{P^{n}_0} \left[ \int_{\Theta} L_n(\theta,\theta_0) d\qrs \right]
        \\
        &\leq \frac{ n M (\e_n^2 + \eta_n^R(\gamma)) }{n \delta M_n (\e_n^2 + \eta_n^R(\gamma))} = \frac{M}{\d M_n},
    \end{align*}   
    where the last inequality follows from Theorem~\ref{thrm:thm1a}. Since $M_n$ is a diverging sequence, convergence in $P^n_0$-probability follows.
    
\end{proof}


\subsection{Proofs in Section~\ref{sbsec:ConditionsL}}

\begin{proof}[Proof of Lemma~\ref{lem:ggv71}:]
    Refer Theorem 7.1 of \cite{GGV}.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:cover}:]	
    For any positive $k$ and $\e$, let $\theta \in [\theta_0 - k\e, \theta_0 + k\e ]^d \subset \Theta \subset \mathbb R^d$. Now consider a set $H_i= \{\theta_i^0,\theta_i^1, \ldots \theta_i^J, \theta_i^{J+1} \}$ and $H=\bigotimes_d H_i $ with $J= \lfloor\frac{2 k\e}{\delta'}\rfloor$, where  $\theta^j_i = \theta_0 - k\e + i\delta'$ for $j=\{0,1,\dots , J \}$ and $\theta_i^{J+1}= \theta_0 + k\e$. Observe that for any $\theta \in [\theta_0 - k\e, \theta_0 + k\e ]^d$, there exists a $\theta^j \in  H$ such that $\| \theta - \theta^j \| < \delta'$. Hence, union of the $\delta'-$balls for each element in set $H$ covers $[\theta_0 - k\e, \theta_0 + k\e ]^d$, therefore $N(\delta',[\theta_0 - k\e, \theta_0 + k\e ]^d, \|\cdot\|) = (J+2)^d$.
    
     %$f(\cdot)$  is locally Lipschitz by Assumption~\ref{assump:Asf4a} and
    %for a given $a\in\sA$,
    % $R(a,\theta)$ is locally Lipschitz in $\theta$ 
     Now, due  to Assumption~\ref{assump:Asf4}, for any $\theta \in [\theta_0 - k\e, \theta_0 + k\e ]^d$
    \begin{align*}
        d_L(\theta,\theta_0) \leq K_2 \| \theta - \theta^j \| \leq K_2 \delta',
    \end{align*}
    %where $C = \sup_{a \in \mathcal{A}} K(a)$ and is finite due to Assumption~\ref{assump:Asf4}. 
    For brevity, we denote $n^{-1} {L_n(\theta,\theta_0)}$ by $d_L(\theta,\theta_0)$, that is
    \vspace{0em}
    \begin{equation}
        d_L(\theta_1,\theta_2) := \sup_{a \in \mathcal{A}} \vert R(a,\theta_1) - R(a,\theta_2) \vert,~ \forall\{\theta_1,\theta_2\}\in\Theta,
        %\label{eq:eqm1}
    \end{equation}
    and the covering number of the set $T(\e):= \{P_{\theta} : d_L(\theta,\theta_0) < \e\}$ as  $N(\delta, T(\e), d_L )$, where $\delta > 0 $ is the radius of each ball in the cover. 
    
    Hence, $\delta'$-cover of set $[\theta_0 - k\e, \theta_0 + k\e ]^d$ is $K_1\delta'$ cover of set $T(\e)$ with $k= 1/K_2$. Finally,
    \begin{align*}
        N(K_2 \delta', T(\e), d_L ) \leq (J+2)^d \leq \left( \frac{2 k\e}{\delta'} + 2 \right)^d=   \left( \frac{2 \e}{K_2\delta'} + 2 \right)^d
    \end{align*}
    
    which implies for $\delta = K_2\delta'$, 
    \begin{align*}
        N(\delta, T(\e), d_L ) \leq  \left(\frac{2 \e}{\delta} + 2 \right)^s.  
    \end{align*}
    %	
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:ass1}:]
    Recall $d_L(\theta,\theta_0) = \left(\sup_{a \in  \mathcal{A}} |R(a,\theta) -  R(a,\theta_0)  |\right)$ and $T(\e)= \{ P_{\theta}: d_L(\theta,\theta_0) < \e \}$. Using Lemma~\ref{lem:cover}, observe that for every $ \e > \e_n > 0$,
    \begin{align*}
        N\left(\frac{\e}{2}, \{ \theta: \e \leq d_L(\theta,\theta_0) \leq 2\e \}, d_L \right) \leq N \left(\frac{\e}{2}, \{ \theta: d_L(\theta,\theta_0) \leq 2\e \}, d_L \right) < 10^d.
    \end{align*}
    Next, using Assumption~\ref{assump:Asf5} we have
    \[ d_L(\theta,\theta_0) \leq  K_1   d_{H}(\theta,\theta_0). \]   
    It follows from the above two observations and Lemma 2 that, for every $\e > \e_n>0$, there exist tests $\{\phi_{n,\e}\}$ such that 
    \begin{align}
        \bbE_{P^{n}_0}[ \phi_{n,\e} ]  &\leq 10^d  \frac{\exp(-C' n \e^2 )}{1-\exp(-C'n\e^2)},  \\
        \underset{\{ \theta\in \Theta : d_L(\theta,\theta_0) \geq \epsilon  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_{n,\e} ] &\leq  \exp(-C' n \e^2 ),\label{eq:eq3}
    \end{align} 
    where $C' = \frac{1}{2 K_1^2}$. Since the above two conditions hold for every $\e > \e_n$, we can choose a constant $K>0$ such that for every $\e >  \e_n$ 
    %> 1 ~ \forall n \geq 1$,
    \begin{align}
        \bbE_{P^{n}_0}[ \phi_{n,\e} ]  &\leq 10^d  \frac{\exp(-C' K^2 n \e^2 )}{1-\exp(-C'K^2n\e^2)} \leq 2 (10^d) \exp(-C' K^2  n \e^2 ), \label{eq:eq2} \\
        \underset{\{ \theta\in \Theta : L_n(\theta,\theta_0) \geq K^2n \e^2  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_{n,\e} ]  & = \underset{\{ \theta\in \Theta : d_L(\theta,\theta_0) \geq K\e  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_{n,\e} ] \leq  \exp(-C' K^2 n \e^2 ),\label{eq:eq31}
    \end{align} 
    %\textcolor{red}{(in Thm 7.1 the original set in~\eqref{eq:eq3} is defined as $ \{ \theta\in \Theta : d(\theta_1,\theta_2) \geq \epsilon \} $)}\\
    where the second inequality in~\eqref{eq:eq2} holds $\forall n \geq n_0$, where $n_0:= \min\{n\geq 1: C' K^2 n \e^2 \geq \log(2)   \}$
    %	\begin{align*}
    %	 \frac{\exp(-C'K^2 n \e_n^2 )}{1-\exp(-C' K^2 n\e_n^2)} &\leq  \exp(-C' n K^2 \e_n^2 ) (1 + \exp(-\tilde{C} n \e_n^2 )) 
    %	\\
    %	&\leq 2 \exp(-C' K^2 n \e_n^2 ),
    %	\end{align*}
    %	
    %	and $n_0$ is the solution of $(1 + \exp(-\tilde{C} n_0 \e^2 )) = \frac{1}{1-\exp(-C' K^2 n_0\e_n^2)}$. 
    Hence, the result follows for $C_1=K^2$ and $C= C' K^2$. 
\end{proof}

%\begin{repeattheorem}[Theorem 1]
%		Let $\e_n$ be a sequence such that $\e_n \to 0$ and $n \e_n^2 \to \infty$ as $n \to \infty$. 
%	%and $$L_n(\theta,\theta_0) = n \left(\sup_{a \in \mathcal{A}} \vert G(a,\theta) - G(a,\theta_0) \vert \right)^2. $$ 
%	Then under Assumptions~\ref{assump:Asf1},~\ref{assump:Asf2},~\ref{assump:Asf3},~\ref{assump:Asf5},~\ref{assump:Asf4} for $C = \frac{C_1}{2(\sup_{a\in \mathcal{A}} K_1(a))^2}$, $C_0= 2*10^s$, $C_1>1$, and positive constants $C_2 $ and $C_3$ such that $C > C_2 + C_3 + 2$, the Naive VB approximation of the true posterior satisfies,
%	\begin{align}
%	\bbE_{P^{n}_0} \left[ \int_{\Theta} L_n(\theta,\theta_0) q^*(\theta| \nX) d\theta \right] \leq M n(\e_n^2 + \gamma_n^2),
%	\label{eq:prop12}
%	\end{align}
%	where constant M depends only on $C,C_0 ,C_1,$ and $\lambda$, and
%	$$ \gamma_n^2 = \frac{1}{n} \inf_{Q \in \sQ} \bbE_{P^{n}_0} [\scKL({q}(\theta)\|\Pi(\theta|\nX)) ].  	$$	
%	%$C_1$ is chosen such that $\sqrt{C_1}\e_n > 1$ and
%	%, and$$ \gamma_n^2 : = \frac{1}{n} \inf_{Q \in \sQ} \bbE_{P^{n}_0} [\scKL({q}(\theta)\|\Pi(\theta|\nX)) ].  	$$	
%\end{repeattheorem}


%\begin{proof}{Proof of Corollary~\ref{corr:cor1}:}
%Using definition of $L_n(\theta,\theta_0)$, Markov inequality,  and \eqref{eq:prop1}, observe that for every $\delta>0$
%%, there exists $M_{\delta} = M/\delta$ such that 
%\begin{align*}
%P^{n}_0\left( \frac{1}{n} \int_{\Theta} L_n(\theta,\theta_0) q^*(\theta| \nX) d\theta > {\delta}  \right) & \leq \frac{\bbE_{P^{n}_0} \left[ \int_{\Theta} L_n(\theta,\theta_0) q^*(\theta| \nX) d\theta \right]}{\delta}
%\\
%& \leq \frac{M (\e_n^2 + \gamma_n^2)}{\delta}.
%\end{align*}
%	\begin{align*}
%			P^{n}_0\left( \frac{1}{\e_n^2 + \gamma_n^2 }\int \left(\sup_{a \in \mathcal{A}} \vert G(a,\theta) - G(a,\theta_0) \vert \right)^2 q^*(\theta| \nX) d\theta > M_n  \right) \leq \frac{M}{M_n} 
%		\end{align*}
%		
%Taking  limit both sides, we get convergence in probability 
%%and if  $\sum_{n\geq 1} (\e_n^2 + \gamma_n^2) < \infty$ , the first Borel-Contelli lemma implies almost sure convergence. 
%\end{proof}
\begin{proof}[Proof of Corollary~\ref{thrm:thm1a}:]
    Using Lemma~\ref{lem:ass1} observe that for any $\Theta_n(\e) \subseteq \Theta$,  $L_n(\theta,\theta_0)$ satisfies Assumption~\ref{assump:Asf1} with $C_0=2* 10^s$, $C = \frac{C_1}{2K_1^2}$ and for any $C_1>0$, since 
    \begin{align*}
        \underset{\{ \theta\in \Theta_n(\e) : L_n(\theta,\theta_0) \geq C_1 n \epsilon_n^2  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_{n,\e} ] \leq \underset{\{ \theta\in \Theta : L_n(\theta,\theta_0) \geq C_1 n \epsilon_n^2 \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_{n,\e} ] &\leq  \exp(-C n \e_n^2 ).
    \end{align*}
    Hence, applying Theorem~\ref{thrm:thm1} the proof follows.
\end{proof}



%\subsection{Proofs in Section~\ref{sbsec:PropEta}}
%
%\begin{proof}[{Proof of Proposition~\ref{prop:prop1}}]
%Fix $\gamma>0$. Now, recall, 
%$\eta_n^R(\gamma) =  \frac{1}{n}\inf_{Q \in \sQ} \bbE_{P^{n}_0} \left[  \scKL(Q(\theta)\|\Pi(\theta|\nX)) 
%- \gamma \inf_{a \in \sA}  \bbE_Q[R(a,\theta)] \right]$. 
%
%For brevity let us denote $ \scKL({q}(\theta)\|\Pi(\theta|\nX))$ as $\scKL$. First, observe that 
%\begin{align} 
%	\nonumber
%	\bbE_{P^{n}_{0}}[\scKL] = \int_{\Theta}& Q(\theta) \log (Q(\theta)) d\theta -
%	\int_{\Theta} Q(\theta) \log
%	d \Pi(\theta) - \bbE_{P^{n}_{0}} \left[ \int_{\Theta} Q(\theta)
%	\log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \right) d\theta \right]
%	\\
%	\label{eq:eqa0a}
%	& + \bbE_{P^{n}_{0}}  \left[ \log \left( \int_{\Theta}   \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}   d\Pi(\theta) \right) \right].
%\end{align}
%Now, using Jensen's inequality and Fubini's theorem in the last term above,
%\begin{align} 
%	\nonumber
%	\bbE_{P^{n}_{0}}  \left[ \log \left( \int_{\Theta}   \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}   d\Pi(\theta) \right) \right] &\leq  \log \left( \bbE_{P^{n}_{0}} \left[ \int_{\Theta}   \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}   d\Pi(\theta) \right] \right)  
%	\\
%	\nonumber
%	&= \log \left(  \int_{\Theta}  \bbE_{P^{n}_{0}}  \left[ \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \right]   d\Pi(\theta)  \right) =0.  
%\end{align}
%Now, substituting the above result into~\eqref{eq:eqa0a} and dividing the third term in~\eqref{eq:eqa0a} over compact set $K$, containing the true parameter $\theta_0$ and its complement in $\Theta$, it follows that
%\begin{align} 
%	\bbE_{P^{n}_{0}}[\scKL] \leq \int_{\Theta}& Q(\theta) \log (Q(\theta)) d\theta -
%	\int_{\Theta} Q(\theta) \log
%	d \Pi(\theta) - \bbE_{P^{n}_{0}} \left[ \int_{K} Q(\theta)
%	\log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \right) d\theta \right] 
%	\nonumber
%	\\
%	&\quad -\bbE_{P^{n}_{0}} \left[ \int_{\Theta \backslash K} Q(\theta)
%	\log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \right) d\theta \right]
%	\label{eq:eqa0}
%\end{align}
%
%Next, we approximate the third term in the previous display using the LAN condition in Assumption~\ref{assume:lan}. Let
%$\Delta_{n,\theta_0} := r_n(\hat{\theta} - \theta_0)$, with $r_n= \sqrt{n}I$. Re-parameterizing the expression with $\theta =
%\theta_0 + r_n^{-1} h$ we have $\int_{K} Q(\theta) \log \left( \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \right)  d\theta $
%\begin{align}
%	\nonumber
%	& = det(r_n)^{-1} \int_{} q(\theta_0 + r_n^{-1}
%	h) \log  \left( \prod_{i=1}^n \frac{p(X_i|(\theta_0  + r_n^{-1} h) )}{p(X_i|\theta_0)} \right)  dh \\
%	\nonumber
%	&= det(r_n)^{-1} \int_{} q(\theta_0 + r_n^{-1} h)
%	\bigg ( h^T
%	I(\theta_0)\Delta_{n,\theta_0} -	\frac{1}{2}h^TI(\theta_0)h+
%	o_{P^n_{\theta_0}}(1) \bigg) dh \\
%	\nonumber
%	&= \int_{K} Q(\theta) \bigg (
%	[r_n(\theta - \theta_0)]^T I(\theta_0)[r_n(\hat \theta - \theta_0)] -
%	\frac{1}{2}  [r_n (\theta - \theta_0)]^T I(\theta_0) [r_n (\theta - \theta_0)] \bigg) d\theta +
%	o_{P^n_{\theta_0}}(1) \\
%	\nonumber
%	&=  - \frac{1}{2}  \int_{K}	Q(\theta)  [r_n (\theta - \hat{\theta})]^TI(\theta_0) [r_n (\theta - \hat{\theta})]  d\theta  + 	\frac{1}{2}  [r_n (\hat \theta - {\theta_0})]^T I(\theta_0) [r_n (\hat \theta - {\theta_0})] \int_{K} dQ(\theta)+ o_{P^n_{\theta_0}}(1)  
%	\\
%	& \geq - \frac{1}{2}  \int_{K}	Q(\theta)  [r_n (\theta - \hat{\theta})]^TI(\theta_0) [r_n (\theta - \hat{\theta})]  d\theta   + o_{P^n_{\theta_0}}(1),  
%	\label{eq:eqa1}
%\end{align}
%where the penultimate equality follows by adding and subtracting  $\frac{1}{2}  [r_n (\hat \theta - {\theta_0})]^T I(\theta_0) [r_n (\hat \theta - {\theta_0})]$ and the last inequality is due to fact that the second term in the penultimate equality is non-negative.
%%On the other hand, using the same re-parametrization calculation we
%%obtain, $ \int_{\Theta}   \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}   d\Pi(\theta) $
%%\begin{align}
%%\nonumber
%%&= n^{-1/2} \int  \pi(\theta_0+ n^{-1/2}h)
%%\prod_{i=1}^n \frac{p(X_i|(\theta_0  + n^{-1/2} h) )}{p(X_i|\theta_0)}  dh\\
%%\nonumber
%%&= e^{o_{P^n_{\theta_0}}(1)} \ n^{-1/2} \int
%%\pi(\theta_0+ n^{-1/2}h) e^{h
%%	I(\theta_0)\Delta_{n,\theta_0} -\frac{1}{2}h^2I(\theta_0)} dh  \\
%%\nonumber
%%&= e^{o_{P^n_{\theta_0}}(1)} e^{\frac{nI(\theta_0)}{2}(\hat{\theta}-\theta_0)^2 } \  \int  \Pi(\theta) e^{-\frac{nI(\theta_0)}{2}(\theta- \hat{\theta})^2 } d\theta.
%%\end{align}
%%Therefore, it follows that
%%\begin{align}
%%\begin{split}\label{eq:eqa2}
%%\log \int_{\Theta} \Pi(\theta) \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} d\theta &= \frac{1}{2} nI(\theta_0) (\hat{\theta}-\theta_0)^2 + \log \int_{\Theta}  \Pi(\theta) e^{-\frac{nI(\theta_0)}{2}(\theta- \hat{\theta})^2 } d\theta  + o_{P^n_{\theta_0}}(1).
%%\end{split}
%%\end{align}
%Now, by substituting equation~\eqref{eq:eqa1}  into~\eqref{eq:eqa0} we obtain,
%\begin{align}
%	\nonumber
%	\bbE_{P^{n}_0}[\scKL] &\leq \int_{\Theta} Q(\theta) \log dQ(\theta) - \int_{\Theta} Q(\theta) \log d \Pi(\theta)  + \frac{1}{2} \bbE_{P^{n}_0} \left[ \int_{K}	Q(\theta)  [r_n (\theta - \hat{\theta})]^T I(\theta_0) [r_n (\theta - \hat{\theta})]  d\theta \right]
%	\\
%	\nonumber 
%	& \quad \quad -\bbE_{P^{n}_{0}} \left[ \int_{\Theta \backslash K} Q(\theta)
%	\log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)} \right) d\theta \right] + \bbE_{P^{n}_0} \left[o_{P^n_{\theta_0}}(1)\right]
%	\\
%	%&=  \scKL(Q(\theta)\| \Pi(\theta)) + \log \int_{\Theta}  \Pi(\theta) e^{-\frac{nI(\theta_0)}{2}(\theta- \hat{\theta})^2 } d\theta  + \frac{1}{2} n  I(\theta_0) \int_{\Theta} ( \theta- \hat{\theta} )^2	Q(\theta)  d\theta  + o_{P^n_{\theta_0}}(1)
%	%\end{align*}
%	%
%	%Now taking expectation with respect to measure $P^n_{\theta_0}$, $\bbE_{P^{n}_0}[\scKL]$
%	%\begin{align}
%	&=  \scKL(Q(\theta)\| \Pi(\theta))  + \frac{1}{2} \int_{K} \bbE_{P^{n}_0} \left[ [r_n (\theta - \hat{\theta})]^T I(\theta_0) [r_n (\theta - \hat{\theta})] \right]	Q(\theta)  d\theta  + \bbE_{P^{n}_0} \left[ o_{P^n_{\theta_0}}(1) \right]
%	\nonumber
%	\\
%	& \quad - \int_{\Theta \backslash K} Q(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta ,
%	\label{eq:eqa3}
%\end{align}
%where the second and fourth terms are due to Fubini's Theorem. Now, using the fact that $\bbE_{P^{n}_0}[ (\theta_0 - \hat{\theta})] = 0$, we have
%\begin{align*}
%	\bbE_{P^{n}_0} &\left[ [r_n (\theta - \hat{\theta})]^T I(\theta_0) [r_n (\theta - \hat{\theta})] \right] 
%	\\
%	&= \bbE_{P^{n}_0} \left[ [r_n (\theta - {\theta_0})]^T I(\theta_0) [r_n (\theta - {\theta_0})] \right] + \bbE_{P^{n}_0} \left[ [r_n (\theta_0 - \hat{\theta})]^T I(\theta_0) [r_n (\theta_0 - \hat{\theta})]\right] 
%	\\
%	& \quad \quad +  2 [r_n (\theta - {\theta_0})]^T I(\theta_0) \left[r_n \bbE_{P^{n}_0} \left[ (\theta_0 - \hat{\theta}) \right] \right] 
%	\\
%	& =  \left[ [r_n (\theta - {\theta_0})]^T I(\theta_0) [r_n (\theta - {\theta_0})] \right] + \bbE_{P^{n}_0} \left[ [r_n (\theta_0 - \hat{\theta})]^T I(\theta_0) [r_n (\theta_0 - \hat{\theta})]\right] .
%\end{align*}
%Substituting the equation above into~\eqref{eq:eqa3}, 
%\begin{align}
%	\nonumber
%	\bbE_{P^{n}_0}[\scKL]& \leq   \frac{1}{2}  \int_{K}  \left[ [r_n (\theta - {\theta_0})]^T I(\theta_0) [r_n (\theta - {\theta_0})] \right]	Q(\theta)  d\theta - \int_{\Theta \backslash K} Q(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta
%	\\
%	&\quad \quad \scKL(Q(\theta)\| \Pi(\theta))   + \frac{1}{2}  \bbE_{P^{n}_0} \left[ [r_n (\theta_0 - \hat{\theta})]^T I(\theta_0) [r_n (\theta_0 - \hat{\theta})]\right] \int_{K} 	Q(\theta)  d\theta +  \bbE_{P^{n}_0} \left[ o_{P^n_{\theta_0}}(1) \right]
%	\nonumber
%	\\
%	& \leq   \frac{1}{2}  \int_{K}  \left[ [r_n (\theta - {\theta_0})]^T I(\theta_0) [r_n (\theta - {\theta_0})] \right]	Q(\theta)  d\theta - \int_{\Theta \backslash K} Q(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta
%	\nonumber
%	\\
%	&\quad \quad \scKL(Q(\theta)\| \Pi(\theta))  + \frac{1}{2}  \bbE_{P^{n}_0} \left[ [r_n (\theta_0 - \hat{\theta})]^T I(\theta_0) [r_n (\theta_0 - \hat{\theta})]\right]  +  \bbE_{P^{n}_0} \left[ o_{P^n_{\theta_0}}(1) \right].
%	\label{eq:eqa4}
%\end{align}
%
%Using~\eqref{eq:eqa4}, it follows that
%\begin{align}
%	\nonumber
%	\bbE_{P^{n}_0} &\left[  \scKL(Q(\theta)\|\Pi(\theta|\nX)) 
%	-  \gamma \inf_{a \in \sA} \bbE_Q[R(a,\theta)] \right]
%	\\
%	\nonumber
%	&\leq  \scKL(Q(\theta)\| \Pi(\theta)) -  \gamma \inf_{a \in \sA} \bbE_Q[R(a,\theta)]  + \frac{1}{2}  \int_{K}  \left[ [r_n (\theta - {\theta_0})]^T I(\theta_0) [r_n (\theta - {\theta_0})] \right]	Q(\theta)  d\theta 
%	\\
%	&\quad  - \int_{\Theta \backslash K} Q(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta + \frac{1}{2}  \bbE_{P^{n}_0} \left[ [r_n (\theta_0 - \hat{\theta})]^T I(\theta_0) [r_n (\theta_0 - \hat{\theta})]\right] +  \bbE_{P^{n}_0} \left[ o_{P^n_{\theta_0}}(1) \right],
%	\label{eq:eqb1}
%\end{align} 
%where matrices $I(\theta_0)$ and $r_n$ are as defined in Assumption~\ref{assume:lan}. Now, it follows from substituting $r_n = \sqrt{n}I$ and the definition of $\eta_n^R(\gamma)$ that,
%\begin{align}
%	\nonumber
%	\eta_n^R (\gamma) & \leq \inf_{Q \in \sQ} \Bigg[ \frac{1}{n} \scKL(Q(\theta)\| \Pi(\theta)) - \frac{\gamma}{n}  \inf_{a \in \sA} \bbE_Q[R(a,\theta)]+ \frac{1}{2}   \int_{K}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [ (\theta - {\theta_0})] \right]	Q(\theta)  d\theta
%	\\
%	& - \frac{1}{n}\int_{\Theta \backslash K} Q(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta  \Bigg]
%	+ \frac{1}{2}  \bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T I(\theta_0) [ (\theta_0 - \hat{\theta})]\right] +  \frac{1}{n}\bbE_{P^{n}_0} \left[ o_{P^n_{\theta_0}}(1) \right].
%	\label{eq:eqb2}
%\end{align}
%
%%Using Cramer-Rao lower bound for $\hat \theta$, we know that $\bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T I(\theta_0) [ (\theta_0 - \hat{\theta})]\right] \leq \frac{1}{n} \bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T Var(\hat \theta)^{-1} [ (\theta_0 - \hat{\theta})]\right]  $  for all $n\geq 1$. Notice that $\left[ [ (\theta_0 - \hat{\theta})]^T Var(\hat \theta)^{-1} [ (\theta_0 - \hat{\theta})]\right]$ is Wald's test statistic and converges in distribution to $\chi^2$ distribution with $d-$degrees of freedom.  It implies that $\bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T Var(\hat \theta)^{-1} [ (\theta_0 - \hat{\theta})]\right]  $ converges to $d$ and thus for large $n $ the fourth term in~\eqref{eq:eqb2} is small. By definition, $\bbE_{P^{n}_0} \left[ o_{P^n_{\theta_0}}(1) \right]$ is small as well, implying that the last two terms on right hand side of~\eqref{eq:eqb2} tends to 0 as $n \to \infty$.
%
%%Observe that the optimization over family $\sQ$ in \eqref{eq:eqb2} above will find a $Q(\theta) \in \sQ$, which is close to the prior $\Pi(\theta)$ in \scKL~divergence and its second moment around $\theta_0$ is atmost the variance of the estimator $\hat{\theta}$.
%
%%Substituting $r_n = \sqrt{n} I$, taking infimum on set $\sQ$ and dividing by $n$, we have 
%%\begin{align}
%%	\nonumber
%%	\frac{1}{n} &\inf_{Q \in \sQ}\bbE_{P^{n}_0}[\scKL] 
%%	\\
%%	\nonumber
%%	&\leq   \inf_{Q \in \sQ} \bigg(   \frac{1}{2}   \int_{K}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [(\theta - {\theta_0})] \right]	Q(\theta)  d\theta - \frac{1}{n}\int_{\Theta \backslash K} Q(\theta)
%%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta
%%	\\
%%	&\quad + \frac{1}{n} \scKL(Q(\theta)\| \Pi(\theta)) \bigg) 
%%	+ \frac{1}{2} \bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T I(\theta_0) [ (\theta_0 - \hat{\theta})]\right]+ \frac{1}{n} \bbE_{P^{n}_0} \left[ o_{P^n_{\theta_0}}(1) \right].
%%	\label{eq:eqa5}	
%%\end{align}
%
%Using Cramer-Rao lower bound for $\hat \theta$, we know that $\bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T I(\theta_0) [ (\theta_0 - \hat{\theta})]\right] \leq \frac{1}{n} \bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T Var(\hat \theta)^{-1} [ (\theta_0 - \hat{\theta})]\right]  $  for all $n\geq 1$. Notice that $\left[ [ (\theta_0 - \hat{\theta})]^T Var(\hat \theta)^{-1} [ (\theta_0 - \hat{\theta})]\right]$ is Wald's test statistic and converges in distribution to $\chi^2$ distribution with $d-$degrees of freedom, implying that 
%\begin{align}
%	\limsup_{n \to \infty} \bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T I(\theta_0) [ (\theta_0 - \hat{\theta})]\right] \leq \limsup_{n \to \infty}  \frac{1}{n} \bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T Var(\hat \theta)^{-1} [ (\theta_0 - \hat{\theta})]\right] = 0.
%\end{align}  
%%It implies that $\bbE_{P^{n}_0} \left[ [ (\theta_0 - \hat{\theta})]^T Var(\hat \theta)^{-1} [ (\theta_0 - \hat{\theta})]\right]  $ converges to $d$ and thus for large $n $ the second term in~\eqref{eq:eqa5} is small. 
%By definition, $\frac{1}{n}\bbE_{P^{n}_0} \left[ o_{P^n_{\theta_0}}(1) \right] \to 0$ as $n \to \infty$.
%% implying that the last two terms on the right hand side of~\eqref{eq:eqa5} tends to 0 as $n \to \infty$.
%
%Next, observe that for any $\hat q_n(\theta)$, that degenerates to $\delta_{\theta_0}$ at the rate of $\sqrt{n}I$, the fist term in~\eqref{eq:eqb2}
%\begin{align}
%	\nonumber
%	 \inf_{Q \in \sQ} \Bigg[ &\frac{1}{n} \scKL(Q(\theta)\| \Pi(\theta)) - \frac{\gamma}{n}  \inf_{a \in \sA} \bbE_Q[R(a,\theta)] + \frac{1}{2}   \int_{K}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [ (\theta - {\theta_0})] \right]	Q(\theta)  d\theta
%	\\
%	\nonumber
%	& - \frac{1}{n}\int_{\Theta \backslash K} Q(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta  \Bigg]
%	\\
%	&\leq  \frac{1}{n} \scKL(\hat q_n(\theta)\| \Pi(\theta)) - \frac{\gamma}{n}  \inf_{a \in \sA} \int_{\Theta}  \hat q_n(\theta) R(a,\theta)	 d\theta+ \frac{1}{2}   \int_{K}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [(\theta - {\theta_0})] \right]	\hat q_n(\theta)  d\theta 
%	\nonumber
%	\\
%	& \quad - \frac{1}{n}\int_{\Theta \backslash K} \hat q_n(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta 
%	\\
%	&= \frac{1}{n} \int_{\Theta} \hat q_n(\theta) \log \hat q_n(\theta) d\theta - \frac{1}{n} \int_{\Theta} \hat q_n(\theta) \log d\Pi(\theta) + \frac{1}{2}   \int_{K}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [(\theta - {\theta_0})] \right]	\hat q_n(\theta)  d\theta 
%	\nonumber
%	\\
%	&\quad - \frac{1}{n}\int_{\Theta \backslash K} \hat q_n(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta - \frac{\gamma}{n}  \inf_{a \in \sA} \int_{\Theta}  \hat q_n(\theta) R(a,\theta)	 d\theta
%	\label{eq:eqb3}	
%	%\label{eq:eqb3}
%\end{align}
%Now, using similar arguments as used in the proof of Proposition~\ref{prop:prop1} and using the fact that $\inf_{a \in \mathcal A} R(a,\theta_0) < \infty$, we can conclude that \( \limsup_{n \to \infty } \eta_n^R \leq 0. \)


%Next, observe that for any $\hat q_n(\theta)$, that degenerates to $\delta_{\theta_0}$ at the rate of $\sqrt{n}I$, the fist term in~\eqref{eq:eqa5}
%\begin{align}
%	\nonumber
%	\inf_{Q \in \sQ} & \left(  \frac{1}{2}   \int_{K}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [(\theta - {\theta_0})] \right]	Q(\theta)  d\theta - \frac{1}{n}\int_{\Theta \backslash K} Q(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta + \frac{1}{n} \scKL(Q(\theta)\| \Pi(\theta)) \right) 
%	\\
%	\nonumber
%	&\leq  \frac{1}{n} \scKL(\hat q_n(\theta)\| \Pi(\theta)) + \frac{1}{2}   \int_{\Theta}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [(\theta - {\theta_0})] \right]	\hat q_n(\theta)  d\theta  - \frac{1}{n}\int_{\Theta \backslash K} Q(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta
%	\\
%	&= \frac{1}{n} \int_{\Theta} \hat q_n(\theta) \log \hat q_n(\theta) d\theta - \frac{1}{n} \int_{\Theta} \hat q_n(\theta) \log d\Pi(\theta) + \frac{1}{2}   \int_{K}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [(\theta - {\theta_0})] \right]	\hat q_n(\theta)  d\theta 
%	\nonumber
%	\\
%	&\quad - \frac{1}{n}\int_{\Theta \backslash K} \hat q_n(\theta)
%	\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta
%	\label{eq:eqa6}
%\end{align}
%Note that, by assumption, $\hat q_n(\theta)$ converges weakly to $\delta_{\theta_0}$. Since, $\log \pi(\theta_0) < \infty$, the second term converges to zero as $n \to \infty$. It is straightforward to observe that the third term also converges to zero as $n \to \infty$ because the compact set $K$ contains the true parameter $\theta_0$ and the last term also converges to zero, since $\inf_{a \in \mathcal A} R(a,\theta_0) < \infty$. Now consider the penultimate term, using Jensen's inequality, $\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] \leq 0$. Combined with the fact that set $\Theta \backslash K$ does not contain true parameter $\theta_0$,
%\[ \liminf_{n \to \infty} \frac{1}{n}\int_{\Theta \backslash K} \hat q_n(\theta)
%\bbE_{P^{n}_{0}} \left[ \log \left(  \prod_{i=1}^n \frac{p(X_i|\theta)}{p(X_i|\theta_0)}  \right) \right] d\theta = 0. \]
%%    therefore the last three terms in the above equation converges to zero as $n \to \infty$. 
%Re-parameterizing the first term in~\eqref{eq:eqb3} by $\mu = r_n(\theta-\theta_0)$ for $r_n= \sqrt{n}I$ and using the definition of the rescaled density $\check {\hat q}_n(\mu) = \frac{1}{det(r_n)}  {\hat q}_n(r_n^{-1} \mu + \theta_0)$,
%\begin{align}
%	\nonumber
%	\frac{1}{n} \int_{\Theta} \hat q_n(\theta) \log \hat q_n(\theta) d\theta & =  \frac{\log det(\sqrt{n}I)}{n}  + \frac{1}{n} \int \check {\hat q}_n(\mu) \log \check {\hat q}_n(\mu) d\mu 
%	\\
%	&= \frac{d}{2} \frac{\log n}{n} + \frac{1}{n} \int \check {\hat q}_n(\mu) \log \check {\hat q}_n(\mu) d\mu 
%\end{align}
%Observe that as $n \to \infty$, $\frac{\log n}{n} \to 0$ and the last term also converges to zero, since  $\int \check {\hat q}_n(\mu) \log \check {\hat q}_n(\mu) d\mu < \infty$. Hence, the above observations combined together imply that 
%\[\limsup_{n \to \infty} \ \eta_n^R(\gamma)  \leq 0.\]
%%Since, $\gamma_n^2$ is always non-negative, we can conclude that $\gamma_n^2$ converges to zero as $n \to \infty$. 
%Since, Theorem~\ref{thrm:thm1} implies that $\e_n^2 + \eta_n^R(\gamma) \geq 0$ for all $n \geq 1$ and $\e_n^2 \to 0$ as $n\to \infty$, it follows that 
%%\vspace{0em}
%\(\lim_{n \to \infty } \eta_n^R(\gamma) = 0. \)


% Observe that the optimization over family $\sQ$ in \eqref{eq:eqa5} above will find a $Q(\theta) \in \sQ$, which is close to the prior $\Pi(\theta)$ in \scKL~divergence and its second moment around $\theta_0$ is atmost the variance of the estimator $\hat{\theta}$.
%$\int_{\Theta}  \left[ [ (\theta - {\theta_0})]^T I(\theta_0) [(\theta - {\theta_0})] \right]	Q(\theta)  d\theta$ is small.
%Observe that
%
%\begin{align}
%\nonumber
%\text{\sc KL} = \int_{\Theta} &Q(\theta) \log dQ(\theta) - \int_{\Theta}    \log ( G(a,\theta) p(\theta) ) dQ(\theta) + \frac{1}{2} \log \left( \frac{2\pi} {n I(\theta)} \right) \\ 
%+  \log \int (G(a,\theta)p(\theta))& \mathcal{N}(\theta;\hat{\theta},(nI(\theta_0))^{-1}) d\theta  + \frac{1}{2}  n  I(\theta_0) \int_{\Theta} (\theta- \hat{\theta})^2	Q(\theta)  d\theta   + o_{P^n_{\theta_0}}(1).
%\label{eqa6}
%%	\\
%%	&= \int_{\Theta} Q(\theta) \log dQ(\theta) - \int_{\Theta}    \log ( G(a,\theta) p(\theta) ) dQ(\theta)  \\ 
%%	&  +  \log \int (G(a,\theta)p(\theta)) \mathcal{N}(\theta;\hat{\theta},(nI(\theta_0))^{-1}) d\theta  -  \int_{\Theta} \log \left(\mathcal{N}(\theta;\hat{\theta},(nI(\theta_0))^{-1})\right) 	Q(\theta)  d\theta   + o_{P^n_{\theta_0}}(1)
%%	\\
%%	&= \int_{\Theta} Q(\theta) \log \frac{Q(\theta)}{\mathcal{N}(\theta;\hat{\theta},(nI(\theta_0))^{-1})} d\theta - \int_{\Theta}    \log ( G(a,\theta) p(\theta) ) dQ(\theta)  \\ 
%%	&  +  \log \int (G(a,\theta)p(\theta)) \mathcal{N}(\theta;\hat{\theta},(nI(\theta_0))^{-1}) d\theta   + o_{P^n_{\theta_0}}(1).
%\end{align}
%
%Let $Q(\theta)$ has mean $\hat \theta$ and variance $\frac{1}{n}$, then by change of variable $\mu = \sqrt{n} (\theta - \hat \theta)$
%\begin{align}
%\int_{\Theta} &Q(\theta) \log dQ(\theta) = \frac{1}{\sqrt{n}}  \int q(\frac{\mu}{\sqrt{n} }+ \hat \theta) \log q(\frac{\mu}{\sqrt{n} }+ \hat \theta)  d \mu = \frac{1}{2} \log n +   \int q_{\mu}(\mu) \log q_{\mu}(\mu)  d \mu.
%\label{eqa5}
%\end{align}
%Substituting ~\eqref{eqa5} in ~\eqref{eqa6}
%\begin{align*}
%\text{\sc KL} =  \int &q_{\mu}(\mu) \log q_{\mu}(\mu)  d \mu - \int_{\Theta}    \log ( G(a,\theta) p(\theta) ) dQ(\theta) + \frac{1}{2} \log \left( \frac{2\pi} {I(\theta)} \right) \\ 
%&  +  \log \int (G(a,\theta)p(\theta)) \mathcal{N}(\theta;\hat{\theta},(nI(\theta_0))^{-1}) d\theta  + \frac{1}{2}   I(\theta_0)   + o_{P^n_{\theta_0}}(1),
%\end{align*}
%where penultimate term in RHS is due to the specific choice of $Q(\theta)$.
%First term is  finite by Assumption~\ref{assume:5} , second term is finite due to Assumption~\ref{assume:2} and ~\ref{assume:3}, and the last term is finite due to Laplace approximation.  	

%\end{proof}

\subsection{Proof of Theorem~\ref{thrm:NV},~\ref{thrm:NVOGvalue}, and ~\ref{thrm:NVOGdecision}}
 
\begin{proof}[Proof of Theorem~\ref{thrm:NV}:]

The proof follows immediately from Theorem~\ref{thrm:thm1} by taking limit $\gamma\to 0^+$ on either side of its main result, that is
\begin{align}
    \bbE_{P^{n}_0} \left[ \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right] \leq M n (\e_n^2  + \eta_n^R(\gamma) ). %\label{eq:lc3}
    %\frac{4 + 4(1+(C_4(\gamma))^{-1})e^{ - \frac{C_11}{2} C_{4}n \e_n^2}}{C_{10}C_{11}(\gamma)},
\end{align}
Fix $n\geq 1$. Now first consider the LHS, use the fact that  for any $a'\in\sA$, $\lim_{\gamma\to 0^+} \qrs = \qnv$, the integrand is also non-negative , and $n\eta_n^{R}(\gamma)<\infty$ due to Proposition~\ref{prop:eta_gamma} (since a decreasing sequence is bounded given $\eta_n^{R}(0)<\infty$), therefore, using Fatou's Lemma we have 
\begin{align}
   \bbE_{P^{n}_0} \left[ \int_{\Theta}  L_n(\theta,\theta_0)\  d \qnv \right] \leq \liminf_{\gamma\to 0^+} \bbE_{P^{n}_0} \left[ \int_{\Theta}  L_n(\theta,\theta_0)\ d\qrs \right]  %\label{eq:lc3}
    %\frac{4 + 4(1+(C_4(\gamma))^{-1})e^{ - \frac{C_11}{2} C_{4}n \e_n^2}}{C_{10}C_{11}(\gamma)},
\end{align}

On the other hand, using similar argument as used in showing $\qrs \to \qnv$ as  $\gamma\to 0^+$, it follows that 
\[ \liminf_{\gamma\to 0^+} \eta_n^{R}(\gamma) = \eta_n^{R}(0).\]
Thus the result follows.








\end{proof}

Next, we obtain a finite sample bound on the regret, defined as the uniform difference between the Naive VB approximate posterior risk and the expected loss under the true data generating measure $P_{0}$. 

\begin{lemma}\label{corr:cor2}
	%For a sequence $M_n \to \infty$ as $n\to \infty$ any $a' \in\sA, \gamma>0$ and for the
	For a constant M as defined in Theorem~\ref{thrm:NV}
	\begin{align}
		\bbE_{P^{n}_0} \left[  \sup_{a \in \mathcal{A}} \left \vert \int    R(a,\theta)  d \qnv - R(a,\theta_0)  \right \vert \right] \leq \left[ M (\e_n^2 + \eta_n(0)) \right]^{\frac{1}{2}}.
	\end{align}
	%	\begin{align}
	%	\lim_{n \to \infty} P^{n}_0\left( \sup_{a \in \mathcal{A}} \left \vert \int   G(a,\theta) q^*(\theta| \nX) d\theta - G(a,\theta_0) \right \vert   > \left[ M_n (\e_n^2 + \gamma_n^2) \right]^{\frac{1}{2}} \right) = 0.
	%		\end{align}
\end{lemma}
%Proof of Corollary~\ref{corr:cor2}:
\begin{proof}
%Fix $a' \in\sA$ and $\gamma>0$. 
The result follows immediately from the following inequalities 
\begin{align*}
	\left( \sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta)  d \qnv - R(a,\theta_0) \right\vert \right)^2 & \leq  \left( \int \sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta_0) \vert   d \qnv \right)^2
	\\
	&\leq \int \left(\sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta_0) \vert \right)^2  d \qnv,
\end{align*}
where the last inequality is  a consequence of Jensens' inequality. Now, using Jensen's inequality again
\vspace{0em} 
\begin{align*}
	&\left ( \bbE_{P^{n}_0} \left[ \sup_{a \in \mathcal{A}} \left \vert \int   R(a,\theta)  d \qnv - R(a,\theta_0) \right \vert \right] \right)^2 
	\\
	&\quad \quad \leq  \bbE_{P^{n}_0} \left[  \left( \sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta)  d \qnv - R(a,\theta_0) \right\vert \right)^2 \right].
\end{align*} 
Now the result follows immediately using Theorem~\ref{thrm:NV}.
\end{proof}

%\begin{proof}{Proof of Theorem~\ref{thrm:NVOGdecision} :}
%The result follows immediately from Lemma~\ref{corr:cor2} and the  following inequality
%\vspace{0em} 
%\begin{align*}
%	\vert V_{q^*} - V_0 \vert \leq  \sup_{a \in \mathcal{A}} \left\vert \int   G(a,\theta)  d \qnv - G(a,\theta_0) \right\vert .
%\end{align*} 
%\end{proof}

\begin{proof}[Proof of Theorem~\ref{thrm:NVOGvalue} and ~\ref{thrm:NVOGdecision} ]

The proof is similar to  Theorem~\ref{thrm:OGValue} and ~\ref{thrm:OGdecision} and hence omitted.
% using Lemma~\ref{corr:cor2}.
%follows immediately from Theorem~\ref{thrm:thm1} by substituting  $R(a,\theta)=0$ and $f(x)=x$. 


\end{proof}

%\begin{proof}[Proof of Corollary~\ref{corr:cor4}:]
%    %The result follows immediately if we show that $\anv=\aos$ and $\gamma^2_n = 0$. 
%    
%    Recall if $\sQ = \sM$, $R(\cdot,\cdot) = 0$, and $f(x)=x$, then it is easy to observe that $\ars$ is the  Bayes posterior risk minimizer, where $\sM$ is large enough to include the true posterior. Therefore, $\ars = \aos$, since $q^*_{\ars,\gamma}(\theta|\nX)$ coincides with the true posterior. Now, observe that, under the above conditions 
%    $\eta_n^R(\gamma)= \frac{1}{n} \inf_{Q \in \sQ} \bbE_{P^{n}_0} \left[  \scKL(Q(\theta)\|\Pi(\theta|\nX)) 
%    \right]$. Since the variational family $\sM$, is large enough to include the true posterior for all $n\geq 1$, there exists a sequence of distributions $\{q'_n(\theta)\} \subset \mathcal{Q}$, such that $\scKL({q'_n}(\theta)\|\Pi(\theta|\nX))=0 \ \forall n \geq 1$. Now, it follows that
%    \begin{align*}
%        \eta_n^R(\gamma) = \frac{1}{n} \inf_{Q \in \sQ}  \bbE_{P^{n}_0}  [\scKL({q}(\theta)\|\Pi(\theta|\nX)) ] \leq \frac{1}{n}  \bbE_{P^{n}_0}  [ \scKL({q'_n}(\theta)\|\Pi(\theta|\nX)) ] =0 \ \forall n \geq 1.
%    \end{align*}
%    %Observe that when the variational family $\mathcal {Q}$ 
%    Since, the \scKL-divergence is always non-negative, the result follows immediately from the above inequality.
%    
%    
%\end{proof}

\subsection{Proof of Theorem~\ref{thrm:LC}, \ref{thrm:LCOGvalue} and~\ref{thrm:LCOGdecision}}

\begin{proof}[Proof of Theorem~\ref{thrm:LC}:]

The proof follows immediately from Theorem~\ref{thrm:LC} by substituting  $\gamma= 1$. %$R(a,\theta)=R(a,\theta)$, and $f(x)=\log(x)$. 


\end{proof}

%Now, recall, $\alc =: \argmin_{a\in\sA} \max_{Q \in \sQ}\left\{ \bbE_q[R(a,\theta)] - \text{KL}(Q(\theta) \| \Pi(\theta|\nX))\right\}.$ To obtain $\alc$ iteratively, we first fix an $a_0\in \sA$ and compute $q^*_{a_0}(\theta| \nX)$ and then solve the outer optimization problem to compute $a_1$.  Similarly, at each iteration $k$, we sequentially update $q^*_{a_k}(\theta| \nX)$ and $a_k$, until convergence. 
% 
Next, we obtain a finite sample bound on the regret as defined in the lemma below:
%, defined as the uniform difference between the naive approximate posterior risk and the expected loss under the true data generating measure $P_{0}$. 

\begin{lemma}\label{corr:cor21}
	Given $\alc \in \mathcal{A}$ and for a constant M, as defined in Theorem~\ref{thrm:LC} 
	\begin{align}
		\bbE_{P^{n}_0} \left[ \sup_{a \in \mathcal{A}} \left \vert \int  \log  G(a,\theta)  dQ^*_{\alc}(\theta| \nX) - R(a,\theta_0) \right \vert \right]  \leq  \left [M (\e_n^2 + \eta_n^{R}(1))\right ]^{\frac{1}{2}}.
	\end{align}
\end{lemma}

%\begin{proof}{Proof of Corollary~\ref{corr:cor11}:}
%	Using definition of $L_n(\theta,\theta_0)$, Markov inequality,  and \eqref{eq:prop3}, observe that for every $\delta>0$
%	%, there exists $M_{\delta} = M/\delta$ such that 
%	\begin{align*}
%	P^{n}_0\left( \frac{1}{n} \int_{\Theta} L_n(\theta,\theta_0) q_{a_0}^*(\theta| \nX) d\theta > {\delta}  \right) & \leq \frac{\bbE_{P^{n}_0} \left[ \int_{\Theta} L_n(\theta,\theta_0) q_{a_0}^*(\theta| \nX) d\theta \right]}{\delta}
%	\\
%	& \leq \frac{M (\e_n^2 + \eta^2_n(a_0))}{\delta}.
%	\end{align*}
%	
%	Taking  limit both sides, we get convergence in probability and if  $\sum_{n\geq 1} (\e_n^2 + \eta^2_n(a_0) ) < \infty$ , the first Borel-Contelli lemma implies almost sure convergence. 
%	%\begin{corollary}\label{corr:cor11}
%	%	Given $a_0 \in \mathcal{A}$ and a sequence $M_n \to \infty$ and $\sum_{n\geq 1} \frac{1}{M_n} < \infty$ 
%	%	\begin{align}
%	%	\int \left(\sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta_0) \vert \right)^2 q^*_{a_0}(\theta| \nX) d\theta \to 0  ,~P_0\text{ - a.s. } 
%	%	\end{align}
%	%\end{corollary}
%	%\begin{proof}
%	%	Using Markov inequality  and Proposition~\ref{prop:prop3},
%	%	\begin{align*}
%	%	P^{n}_0\left( \int \left(\sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta_0) \vert \right)^2 q^*_{a_0}(\theta| \nX) d\theta > M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0)) \right) \leq \frac{M}{M_n}.
%	%	\end{align*}
%	%	
%	%	Taking  limit both sides we get convergence in probability. Since $\sum_{n\geq 1} \frac{1}{M} < \infty$ , the first Borel-Contelli lemma implies almost sure convergence.
%\end{proof}

\begin{proof}
First, observe that
\begin{align*}
	\left( \sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta) dQ_{\alc}^*(\theta| \nX)  - R(a,\theta_0) \right\vert \right)^2 & \leq 
	\left( \int \sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta_0) \vert   dQ^*_{\alc}(\theta| \nX) \right)^2
	\\
	&	\leq \int \left(\sup_{a \in \mathcal{A}} \vert R(a,\theta) - R(a,\theta_0) \vert \right)^2  dQ^*_{\alc}(\theta| \nX),
\end{align*}
where the last inequality follows from Jensen's inequality. Now, using the Jensen's inequality again 
\begin{align*}
	& \left ( \bbE_{P^{n}_0} \left[ \sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta) dQ_{\alc}^*(\theta| \nX)  - R(a,\theta_0) \right\vert \right] \right)^2 
	\\ 
	& \quad \quad \leq  \bbE_{P^{n}_0} \left[  \left( \sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta) dQ_{\alc}^*(\theta| \nX)  - R(a,\theta_0) \right\vert \right)^2 \right].
\end{align*}
Now, using Theorem~\ref{thrm:LC} for $a_0 = \alc$, the result follows immediately.

\end{proof}

\begin{proof}{Proof of Theorem~\ref{thrm:LCOGvalue}~and~\ref{thrm:LCOGdecision}}: The proof is similar to  Theorem~\ref{thrm:OGValue} and ~\ref{thrm:OGdecision} and hence omitted. 

	
%	%Now, suppose that for a given $\e>0 $, $\sup_{a \in \mathcal{A}} \left\vert \int   G(a,\theta) q^*(\theta| \nX) d\theta - G(a,\theta_0) \right\vert \leq \e$. Then for $\anv \in \underset{z \in \mathcal{A} }{\arg \min} \int   G(z,\theta) q^*(\theta| \nX) d\theta  $, it follows from the definition of $\Psi(\cdot)$ that
%	%\begin{align*}
%	%	\Psi&\left( d(\anv, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) ) \right) 
%	%	\\
%	%	&\leq G( \anv,\theta_0) - \inf_{z \in \mathcal{A}} G(z,\theta_0) 
%	%	\\
%	%	%& = \vert  G( \anv,\theta_0) - \inf_{z \in \mathcal{A}} G(z,\theta_0)  \vert 
%	%	%\\
%	%	& =  G( \anv,\theta_0) - \int   G(\anv,\theta) q^*(\theta| \nX) d\theta   +   \int   G(\anv,\theta) q^*(\theta| \nX) d\theta  - \inf_{z \in \mathcal{A}} G(z,\theta_0)  
%	%	\\
%	%	& \leq  \left \vert  G( \anv,\theta_0) - \int   G(\anv,\theta) q^*(\theta| \nX) d\theta   \right \vert + \left \vert  \int   G(\anv,\theta) q^*(\theta| \nX) d\theta  - \inf_{z \in \mathcal{A}} G(z,\theta_0)  \right \vert 
%	%	\\
%	%	& \leq 2 \sup_{a \in \mathcal{A}} \left\vert \int   G(a,\theta) q^*(\theta| \nX) d\theta - G(a,\theta_0) \right\vert \leq 2\e. 
%	%\end{align*}
%	%
%	%%Since $\Psi(\cdot)$ is strictly increasing, 
%	%Substituting $\e = \left[ M (\e_n^2 + \gamma_n^2) \right]^{\frac{1}{2}}$
%	%\begin{align*}
%	%	& P^{n}_0\left( \Psi\left (d(\anv, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) ) \right)   > 2 \left[ M_n (\e_n^2 + \gamma_n^2) \right]^{\frac{1}{2}} \right) 
%	%	\\
%	%	& \leq  P^{n}_0 \left( \sup_{a \in \mathcal{A}} \left \vert \int   G(a,\theta) q^*(\theta| \nX) d\theta - G(a,\theta_0) \right \vert   > \left[ M_n (\e_n^2 + \gamma_n^2) \right]^{\frac{1}{2}} \right). 
%	%\end{align*}
%	%Next using Corollary~\ref{corr:cor2} it follows immediately  for a diverging sequence $M_n$ that
%	%\begin{align*}
%	%%&\lim_{n \to \infty} P^{n}_0\left( \Psi\left (d(\anv, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) ) \right)   > 2 M_n (\e_n^2 + \gamma_n^2) \right) = 0 \\
%	%&\lim_{n \to \infty} P^{n}_0\left( \Psi\left (d(\anv, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) ) \right)   \leq 2 \left[ M_n (\e_n^2 + \gamma_n^2) \right]^{\frac{1}{2}} \right) = 1. 
%	%\end{align*}
%	%
%	%Observe that for large $n$ using the consistency of $\anv$ and
%	%for any $\tau >0$ such that $C-\tau > 0$, the following inequality holds due to the property of growth function, that is $\lim_{d \to 0} \Psi(d)/d^{\delta} = C$,
%	%\begin{align}
%	%P^{n}_0\left( \Psi\left (d(\anv, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) ) \right)   \leq 2 \left[ M_n (\e_n^2 + \gamma_n^2) \right]^{\frac{1}{2}} \right) \leq P^{n}_0\left( C-\tau \leq   \frac {2 \left[ M_n (\e_n^2 + \gamma_n^2) \right]^{\frac{1}{2}}}{(d(\anv, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) ))^{\delta}} \right). \label{eq:gr1}
%	%\end{align} 
%	%
%	%Since $\tau$ can be made arbitrarily small, taking limits on both sides of~\eqref{eq:gr1}
%	%\begin{align*}
%	%\lim_{n \to \infty} P^{n}_0\left( d(\anv, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) )    \leq  \left[\frac{2 \left[ M_n (\e_n^2 + \gamma_n^2) \right]^{\frac{1}{2}}}{C} \right]^\frac{1}{\delta} \right) = 1.
%	%\end{align*} 
%	%
%	%\textit{Finite sample result}
%	
%	For any $\tau>0$, observe that the result in Lemma~\ref{corr:cor21} implies that $P_0^n-$ probability of 
%	\begin{align}
%		\left\{ \left[ M (\e_n^2 + \eta_n^{R}(1)) \right]^{-\frac{1}{2}} \sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta) q_{\alc}^*(\theta| \nX) d\theta -R(a,\theta_0) \right\vert > \tau \right\}
%	\end{align}
%%\in \underset{z \in \mathcal{A} }{\arg \min} \int   G(z,\theta) q^*(\theta| \nX) d\theta  $
%	is at most $\tau^{-1}$. For $\alc$, it follows from the definition of $\Psi^{\log}(\cdot)$ that
%	\begin{align}
%		\nonumber
%		\Psi^{\log}&\left( d_h(\alc, \underset{z \in \mathcal{A} }{\arg \min}   ~ R(z,\theta_0) ) \right) 
%		\\
%		\nonumber
%		&\leq R( \alc,\theta_0) - \inf_{z \in \mathcal{A}} R(z,\theta_0) 
%		\\
%		\nonumber
%		%& = \vert  G( \alc,\theta_0) - \inf_{z \in \mathcal{A}} G(z,\theta_0)  \vert 
%		%\\
%		& =  R( \alc,\theta_0) - \int   R(\alc,\theta) q_{\alc}^*(\theta| \nX) d\theta   +   \int   R(\alc,\theta) q_{\alc}^*(\theta| \nX) d\theta  - \inf_{z \in \mathcal{A}} R(z,\theta_0)  
%		\\
%		\nonumber
%		& \leq  \left \vert  R( \alc,\theta_0) - \int   R(\alc,\theta) q_{\alc}^*(\theta| \nX) d\theta   \right \vert + \left \vert  \int   R(\alc,\theta) q_{\alc}^*(\theta| \nX) d\theta  - \inf_{z \in \mathcal{A}} R(z,\theta_0)  \right \vert 
%		\\
%		& \leq 2 \sup_{a \in \mathcal{A}} \left\vert \int  R(a,\theta) q_{\alc}^*(\theta| \nX) d\theta - R(a,\theta_0) \right\vert. 
%		\label{eq:eqt2}
%	\end{align}
%	It follows from the above inequality that
%	\begin{align}
%		\nonumber
%		\bigg\{ \left[ M (\e_n^2 + \eta_n^{R}(1)) \right]^{-\frac{1}{2}} \Psi^{\log}\bigg( &d_h(\alc, \underset{z \in \mathcal{A} }{\arg \min}   ~ R(z,\theta_0) ) \bigg) > 2 \tau \bigg\}
%		\\
%		& \subseteq \left\{ \left[ M (\e_n^2 + \eta_n^{R}(1)) \right]^{-\frac{1}{2}} \sup_{a \in \mathcal{A}} \left\vert \int  R(a,\theta) q_{\alc}^*(\theta| \nX) d\theta - R(a,\theta_0) \right\vert > \tau \right\} .
%		\label{eq:eq32a}
%	\end{align} 
%	Therefore, using the condition on the growth function in the statement of the theorem that, $\frac{\Psi^{\log}\left(d_h\left(\alc, \underset{z \in \mathcal{A} }{\arg \min}   ~ R(z,\theta_0) \right)\right)}{d_h\left(\alc, \underset{z \in \mathcal{A} }{\arg \min}   ~ R(z,\theta_0) \right)^{\delta}} = C^{\log},$ the $P_0^n-$ probability of the following event is at least $ 1- \tau^{-1}$:
%	\begin{align}
%		\bigg\{    d_h(\alc, \underset{z \in \mathcal{A} }{\arg \min}   ~ R(z,\theta_0) )  \leq \tau^{\frac{1}{\delta}} \left[ \frac{2 \left[ M (\e_n^2 + \eta_n^{R}(1)) \right]^{\frac{1}{2}} }{C^{\log}} \right]^{\frac{1}{\delta}} \bigg\}.
%	\end{align}
%	Using the monotonicity of logarithm function, it follows that $\underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) = \underset{z \in \mathcal{A} }{\arg \min}  ~ G(z,\theta_0) $ and hence the result follows.
	% %substituting~\eqref{eq:eqt2} into~\eqref{eq:eqt1} that
	%\begin{align}
	%	d(\alc, \underset{z \in \mathcal{A} }{\arg \min}   ~ G(z,\theta_0) )^{\delta} \leq \left[ \frac{2 \sup_{a \in \mathcal{A}} \left\vert \int   G(a,\theta) q^*(\theta| \nX) d\theta - G(a,\theta_0) \right\vert}{C- \phi(t)} \right]
	%	\end{align}

%	Since we know that $\alc$ is consistent and thus for $a_0= \alc$, using similar techniques as used in the corresponding Proposition~\ref{prop:prop2} in the Naive VB case, 
%	\begin{align*}
%	\lim_{n \to \infty} P^{n}_0\left( d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~R(z,\theta_0) )    > \left[\frac{2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(\alc))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \right) = 0.
%	\end{align*}
%	Now observe that 
%	\begin{align*}
%	P^{n}_0\left( d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~R(z,\theta_0) )    > \left[\frac{2 \left [M_n (\e_n^2 + \sup_{a \in \mathcal{A} }\eta_n^{R}(1)^2(a))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \right) 
%	\\
%	\leq 	P^{n}_0\left( d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~R(z,\theta_0) )    > \left[\frac{2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(\alc))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \right).
%	\end{align*}
%	This concludes the proposition.
	%	First observe that for any $\e>0 $, if $\sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta) q^*_{a_0}(\theta| \nX) d\theta - R(a,\theta_0) \right\vert \leq \e$, then for any $\alc \in \underset{z \in \mathcal{A} }{\arg \min} \int   R(z,\theta) q^*_{a_0}(\theta| \nX) d\theta  $, it follows from the definition of $\Psi^{\log}(\cdot)$ 
	%	\begin{align*}
	%	\Psi^{\log}\left( d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) ) \right)  &\leq R( \alc,\theta_0) - \inf_{z \in \mathcal{A}} R(z,\theta_0) 
	%	\\
	%	& = \vert \log  G( \alc,\theta_0) - \inf_{z \in \mathcal{A}} R(z,\theta_0)  \vert 
	%	\\
	%	& \leq \left \vert  R( \alc,\theta_0) - \int   R(\alc,\theta) q^*_{a_0}(\theta| \nX) d\theta   \right \vert + 
	%	\\
	%	& \quad \quad \left \vert  \int   R(\alc,\theta) q^*_{a_0}(\theta| \nX) d\theta  - \inf_{z \in \mathcal{A}} R(z,\theta_0)  \right \vert 
	%	\\
	%	& \leq 2 \sup_{a \in \mathcal{A}} \left\vert \int   R(a,\theta) q^*_{a_0}(\theta| \nX) d\theta - R(a,\theta_0) \right\vert \leq 2\e. 
	%	\end{align*}
	%	
	%	Since $\Psi^{\log}(\cdot)$ is strictly increasing, substituting $\e = M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0) )$
	%	\begin{align*}
	%	& P^{n}_0\left( \Psi^{\log}\left (d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) ) \right)   > 2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0))\right ]^{\frac{1}{2}} \right) 
	%	\\
	%	& \leq  P^{n}_0 \left( \sup_{a \in \mathcal{A}} \vert \int   R(a,\theta) q^*_{a_0}(\theta| \nX) d\theta - R(a,\theta_0) \vert   > M_n ( \e_n^2 + \eta_n^{R}(1)^2(a_0)) \right) 
	%	\end{align*}
	%	
	%	Next using Corollary~\ref{corr:cor21} it follows immediately  for a diverging sequence $M_n$ that
	%	\begin{align*}
	%	\lim_{n \to \infty} P^{n}_0\left( \Psi^{\log}\left (d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) ) \right)   > 2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0))\right ]^{\frac{1}{2}} \right) = 0.
	%	\end{align*}
	%	
	%	Hence for large $n$ using the consistency of $\alc$ and the property of growth function, that is $\lim_{d \to 0} \Psi^{\log}(d)/d^{\delta} = \tilde{C}$, it follows that 
	%	\begin{align*}
	%	\lim_{n \to \infty} P^{n}_0\left( d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) )    > \left[\frac{2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \right) = 0.
	%	\end{align*}
\end{proof}

%\begin{proof}{Proof of Theorem~\ref{prop:prop4}(2):} The proof follows similar steps till equation~\eqref{eq:eq32a} in the proof above and then uses the condition on the growth function $\Psi^{\log}(\cdot)$ given in the statement of the theorem for all $n\geq n_0$. 
%
%
%\end{proof}

%\begin{proof}{Proof of Corollary~\ref{corr:cor41}:}
%	%	Using triangular inequality it is straightforward to see that
%	%	
%	%	\begin{align*}
%	%	& P^{n}_0\left( d(\aos, \alc)     > 2\left[\frac{2 M_n \e_n^2}{{C}} \right]^\frac{1}{\delta} + 2\left[\frac{2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \right)
%	%	\\
%	%	&\leq P^{n}_0\bigg( d(\aos, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) ) + d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) )     
%	%	\\
%	%	& \quad \quad \quad \quad > 2\left[\frac{2 M_n \e_n^2}{{C}} \right]^\frac{1}{\delta} +2 \left[\frac{2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \bigg)
%	%	\\
%	%	&\leq P^{n}_0\left( d(\aos, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) )     > \left[\frac{2 M_n \e_n^2}{{C}} \right]^\frac{1}{\delta} + \left[\frac{2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \right)
%	%	\\
%	%	& \quad+
%	%	P^{n}_0\left(  d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) )     > \left[\frac{2 M_n \e_n^2}{{C}} \right]^\frac{1}{\delta} + \left[\frac{2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \right)
%	%	\\
%	%	& \leq P^{n}_0\left( d(\aos, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) )     > \left[\frac{2 M_n \e_n^2}{{C}} \right]^\frac{1}{\delta}  \right) 
%	%	\\
%	%	& \quad +
%	%	P^{n}_0\left(  d(\alc, \underset{z \in \mathcal{A} }{\arg \min}  ~ R(z,\theta_0) )     >  \left[\frac{2 \left [M_n (\e_n^2 + \eta_n^{R}(1)^2(a_0))\right ]^{\frac{1}{2}}}{\tilde{C}} \right]^\frac{1}{\delta} \right)
%	%	\end{align*}
%	%	
%	The proof follows immediately using triangular inequality, Corollary~\ref{corr:cor41}, Theorem~\ref{prop:prop4}, and using the monotonicity of logarithmic function. 
%\end{proof}

\input{NewsVendor2.tex}

\subsection{Gaussian process classification}

\begin{proof}[Proof of Lemma~\ref{lem:gp2}]
    In view of Theorem~7.1 in~\cite{GGV}, it suffices to show that 
     \[N\left( \e, \Theta_n(\e),d_\text{TV} \right) \leq e^{\bar C n\e^2},\] for some $\bar C>0$. Now, first observe that 
     \begin{align}
         \nonumber
         d_{\text{TV}}(P_{\theta(y)},P_{\theta_0(y)}) &= \frac{1}{2} \bbE_{\nu}\left( |\Psi_1(\theta(y))-\Psi_1(\theta_0(y)) |  + |\Psi_{-1}(\theta(y))-\Psi_{-1}(\theta_0(y)) | \right)
         \\
         \nonumber
         &=  \bbE_{\nu}\left( |\Psi_1(\theta(y))-\Psi_1(\theta_0(y)) |  \right)
         \\
         &\leq \bbE_{\nu}\left( |\theta(y)-\theta_0(y) |  \right) \leq \|\theta(y)-\theta_0(y) \|_{\infty}, 
         \end{align}
    where the second equality uses the definition of $\Psi_{-1}(\cdot)$. Since, total-variation distance is bounded above by supremum norm, hence there exists  a constant $0<c'<1/2$, such that
      \begin{align}
          N\left( \e, \Theta_n(\e),d_\text{TV} \right) \leq N\left( c'\e, \Theta_n(\e),\|\cdot\|_{\infty} \right) \leq  e^{\frac{2}{3} c'^2 C_{10}n\e^2},
          \end{align}
      where the last inequality follows from~\eqref{eq:testGP} in Lemma~\ref{lem:GP}. 
    Then if follows from Theorem~7.1 in~\cite{GGV} that for every $\e> \e_n$, there exists a test $\phi_n$ (depending on $\e>0$) such that, for every $j\geq 1$,
    %a universal constant $K$ and
    %\vspace{1em}
    \begin{align*}
        \bbE_{P^{n}_0}[ \phi_n ]  &\leq e^{\frac{2}{3} c'^2 C_{10}n\e^2} e^{ -\frac{1}{2}n \e^2 }\frac{1}{1-\exp \left (-\frac{1}{2} n\e^2 \right)}, \text{and}\\
        \underset{\{ \theta\in \Theta_n(\e)  : d_{TV}(P_{\theta},P_{\theta_0}) > j \e  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_n ] &\leq  \exp\left(- \frac{1}{2} n \e^2 j\right).
    \end{align*} 
    Now for all $n$ such that $n\e^2>n\e_n^2>2\log2$ and $C_{10}=c'^{-2}/4>1$ and $j=1$, we have
    \begin{align}
        \label{eq:eqt1}
        \bbE_{P^{n}_0}[ \phi_n ]  &\leq 2  e^{ -\frac{1}{3}n \e^2 }, \text{and}\\
        \underset{\{ \theta\in \Theta_n(\e)  : d_{TV}(P_{\theta},P_{\theta_0}) >  \e  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_n ] 
        &\leq  e^{- \frac{1}{2} n \e^2 }\leq e^{ -\frac{1}{3}n \e^2 } .
        \label{eq:eqt2}
    \end{align} 
    
    Now observe that 
    \begin{align}
        \nonumber
        \sup_{a \in \mathcal{A}} | G(a,\theta) - G(a,\theta_0)  | &= \max\left(  c_+ |\bbE_{\nu}[\Psi_{-1}(\theta(y))] -\bbE_{\nu}[\Psi_{-1}(\theta_0(y))] |   , c_- |\bbE_{\nu}[\Psi_{1}(\theta(y))] -\bbE_{\nu}[\Psi_{1}(\theta_0(y))] |\right) 
        \\
        \nonumber
        &= \max\left(  c_+ |\bbE_{\nu}[\Psi_{1}(\theta_0(y))] -\bbE_{\nu}[\Psi_{1}(\theta(y))] |   , c_- |\bbE_{\nu}[\Psi_{1}(\theta(y))] -\bbE_{\nu}[\Psi_{1}(\theta_0(y))] |\right) 
        \\
        \nonumber
        &= \max(c_+,c_-)|\bbE_{\nu}[\Psi_{1}(\theta_0(y))] -\bbE_{\nu}[\Psi_{1}(\theta(y))] |
        \\
        \nonumber
        &\leq \max(c_+,c_-)\bbE_{\nu}[|\Psi_{1}(\theta_0(y)) -\Psi_{1}(\theta(y))| ]
        \\
        %\nonumber
        &\leq  \max(c_+,c_-)d_{TV}(P_{\theta},P_{\theta_0})
        %\\
        %&\leq \max(c_+,c_-)\|\theta_0(y) -\theta(y) \|_{\infty},
        %\\
        %&=\max(c_+,c_-)\|\Psi_{1}(\theta_0(y)) -\Psi_{1}(\theta(y)) \|_{\infty}
        %\\
        %&\leq C_{11}\max(c_+,c_-) d_H(P_{\theta},P_{\theta_0}),
        % &\leq C_{11}\max(c_+,c_-) d_H(P_{\theta},P_{\theta_0}), %\max(c_+,c_-)\bbE_{\nu}[|\Psi_{1}(\theta_0(y)) -\Psi_{1}(\theta(y))| ] \leq 1/\sqrt{2\pi} \max(c_+,c_-)\|\theta_0(y) -\theta(y)\|_{\nu,1} ,
    \end{align} 
    where the second equality uses the fact that $\Psi_{-1}(\cdot)= 1-\Psi_{1}(\cdot)$.%, and the penultimate inequality follows since $\psi_{1}(\cdot)$ is uniformly bounded  by 1.
     Consequently,
    \[ \{ \theta\in \Theta_n(\e)  : \sup_{a \in \mathcal{A}} | G(a,\theta) - G(a,\theta_0)  | > { \max(c_+,c_-)\e} \} \subseteq \{ \theta\in \Theta_n(\e)  : d_{TV}(P_{\theta},P_{\theta_0}) >  \e  \} \] Therefore, it follows from~\eqref{eq:eqt1} and~\eqref{eq:eqt2} and the  definition of $L_n(\theta,\theta_0)$ that 
    \begin{align}
        \bbE_{P^{n}_0}[ \phi_n ]  &\leq 2  e^{ -\frac{1}{3}n \e^2 }, \text{and}\\
        \underset{\{ \theta\in \Theta_n(\e)  : L_n(\theta,\theta_0) > ( \max(c_+,c_-))^2 n \e^2  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_n ] 
        &\leq  e^{- \frac{1}{2} n \e^2 }\leq e^{ -\frac{1}{3}n \e^2 } .
    \end{align} 
    
    Finally, the result follows for $C=1/3$, $C_0=2$ and $C_1= (\max(c_+,c_-))^2$.
    
%    Fix the norm on $\Theta$ to to be the supremum norm, denoted as $\|\cdot\|_{\infty}$. Now observe that the result in~\eqref{eq:testGP} implies that for every $\e > \e_n$,
%    %\vspace{0em}
%    \begin{align*} 
%        N\left( \e/2, \left\{ \theta \in \Theta_n(\e/6): \e \leq \|\theta-\theta_0\|_{\infty} \leq 2\e , \|\cdot\|_{\infty}\right\}  \right) %&\leq  N\left( \e/2, \left\{ P_{\theta}:  d_{H}(P_{\theta},P_{\theta_0}) \leq 2\e \right\} ,d_H \right)
%        %\\
%        & \leq  N\left( \frac{\e}{2}, \Theta_n(\e/6),\|\cdot\|_{\infty} \right) \leq e^{C_{10}/6n\e^2},
%    \end{align*}
%    %where $\Theta_n(2\e)= \{d_{H}(P_{\theta},P_{\theta_0})<2\e\}\cup \{\|\theta-\theta_0\|_{\bbH}<M_n\} $ for some sequence $M_n$ 
%    (refer proof of Theorem 2.1~\cite{Zanten08} for the defintion of $\Theta_n(\e)$).
%    %\vspace{-0.5em}
%    Then if follows from Theorem~7.1 in~\cite{GGV} that for every $\e> \e_n$, there exists a test $\phi_n$ (depending on $\e>0$) such that, for every $j\geq 1$,
%    %a universal constant $K$ and
%    %\vspace{1em}
%    \begin{align*}
%        \bbE_{P^{n}_0}[ \phi_n ]  &\leq e^{C_{10}/6n\e^2} e^{ -\frac{1}{2}n \e^2 }\frac{1}{1-\exp \left (-\frac{1}{2} n\e^2 \right)}, \text{and}\\
%        \underset{\{ \theta\in \Theta_n(\e)  : \|\theta-\theta_0\|_{\infty} > j \e  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_n ] &\leq  \exp\left(- \frac{1}{2} n \e^2 j\right).
%    \end{align*} 
%    Now for all $n$ such that $n\e^2>n\e_n^2>2\log2$ and $C_{10}=2$ and $j=1$, we have
%    \begin{align}
%        \label{eq:eqt1}
%        \bbE_{P^{n}_0}[ \phi_n ]  &\leq 2  e^{ -\frac{1}{6}n \e^2 }, \text{and}\\
%        \underset{\{ \theta\in \Theta_n(\e)  : \|\theta-\theta_0\|_{\infty} >  \e  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_n ] 
%        &\leq  e^{- \frac{1}{2} n \e^2 }\leq e^{ -\frac{1}{6}n \e^2 } .
%        \label{eq:eqt2}
%    \end{align} 
%    
%    Now observe that 
%    \begin{align}
%        \nonumber
%        \sup_{a \in \mathcal{A}} | G(a,\theta) - G(a,\theta_0)  | &= \max\left(  c_+ |\bbE_{\nu}[\Psi_{-1}(\theta(y))] -\bbE_{\nu}[\Psi_{-1}(\theta_0(y))] |   , c_- |\bbE_{\nu}[\Psi_{1}(\theta(y))] -\bbE_{\nu}[\Psi_{1}(\theta_0(y))] |\right) 
%        \\
%        \nonumber
%        &= \max\left(  c_+ |\bbE_{\nu}[\Psi_{1}(\theta_0(y))] -\bbE_{\nu}[\Psi_{1}(\theta(y))] |   , c_- |\bbE_{\nu}[\Psi_{1}(\theta(y))] -\bbE_{\nu}[\Psi_{1}(\theta_0(y))] |\right) 
%        \\
%        \nonumber
%        &= \max(c_+,c_-)|\bbE_{\nu}[\Psi_{1}(\theta_0(y))] -\bbE_{\nu}[\Psi_{1}(\theta(y))] |
%        \\
%        \nonumber
%        &\leq \max(c_+,c_-)\bbE_{\nu}[|\Psi_{1}(\theta_0(y)) -\Psi_{1}(\theta(y))| ]
%        \\
%        \nonumber
%        &\leq  \max(c_+,c_-)\bbE_{\nu}[|\theta_0(y) -\theta(y)| ]
%        \\
%        &\leq \max(c_+,c_-)\|\theta_0(y) -\theta(y) \|_{\infty},
%        %\\
%        %&=\max(c_+,c_-)\|\Psi_{1}(\theta_0(y)) -\Psi_{1}(\theta(y)) \|_{\infty}
%        %\\
%        %&\leq C_{11}\max(c_+,c_-) d_H(P_{\theta},P_{\theta_0}),
%        % &\leq C_{11}\max(c_+,c_-) d_H(P_{\theta},P_{\theta_0}), %\max(c_+,c_-)\bbE_{\nu}[|\Psi_{1}(\theta_0(y)) -\Psi_{1}(\theta(y))| ] \leq 1/\sqrt{2\pi} \max(c_+,c_-)\|\theta_0(y) -\theta(y)\|_{\nu,1} ,
%    \end{align} 
%    where the second equality uses the fact that $\Psi_{-1}(\cdot)= 1-\Psi_{1}(\cdot)$, and the penultimate inequality follows since $\psi_{1}(\cdot)$ is uniformly bounded  by 1. Consequently,
%    \[ \{ \theta\in \Theta_n(\e)  : \sup_{a \in \mathcal{A}} | G(a,\theta) - G(a,\theta_0)  | > { \max(c_+,c_-)\e} \} \subseteq \{ \theta\in \Theta_n(\e)  : \|\theta_0(y) -\theta(y) \|_{\infty} >  \e  \} \] Therefore, it follows from~\eqref{eq:eqt1} and~\eqref{eq:eqt2} and the  definition of $L_n(\theta,\theta_0)$ that 
%    \begin{align}
%        \bbE_{P^{n}_0}[ \phi_n ]  &\leq 2  e^{ -\frac{1}{3}n \e^2 }, \text{and}\\
%        \underset{\{ \theta\in \Theta_n(\e)  : L_n(\theta,\theta_0) > (C_{11} \max(c_+,c_-))^2 n \e^2  \}}{\sup} \bbE_{P^{n}_{\theta}}[ 1- \phi_n ] 
%        &\leq  e^{- \frac{1}{2} n \e^2 }\leq e^{ -\frac{1}{3}n \e^2 } .
%    \end{align} 
%    
%    Finally, the result follows for $C=1/6$, $C_0=2$ and $C_1= (\max(c_+,c_-))^2$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:gp3}]
    The R\'enyi divergence 
    \begin{align*}
        D_{1+\lambda}(P_0^n\| P_{\theta}^n) &=  n \frac{1}{\lambda} \ln \int \left( \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{-\lambda} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{-\lambda}  \right) \nu(dy)
        \\
        &= n \frac{1}{\lambda} \ln \int e^{\lambda \frac{1}{\lambda}\ln \left( \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{-\lambda} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{-\lambda}  \right) } \nu(dy).
        %    \\
        %    &\leq n \frac{1}{\lambda} \ln \int e^{\lambda \ln \left(1+ \frac{|\Psi_{1}(\theta_0(y))-\Psi_{1}(\theta(y)) |}{\min(\Psi_{1}(\theta(y)),\Psi_{-1}(\theta(y)))}\right) } \nu(dy)
        %    \\
        %    &\leq n \frac{1}{\lambda} \ln \int e^{\lambda \left(\frac{|\Psi_{1}(\theta_0(y))-\Psi_{1}(\theta(y)) |}{\min(\Psi_{1}(\theta(y)),\Psi_{-1}(\theta(y)))}\right) } \nu(dy)
        %    \\
        %    &\leq n \frac{1}{\lambda} \ln \int e^{\lambda \left(\sup_{y\in \bbR^d}\frac{|\Psi_{1}(\theta_0(y))-\Psi_{1}(\theta(y)) |}{\min(\Psi_{1}(\theta(y)),\Psi_{-1}(\theta(y)))}\right) } \nu(dy)
        %    \\
        %    &= n \sup_{y\in \bbR^d}\frac{|\Psi_{1}(\theta_0(y))-\Psi_{1}(\theta(y)) |}{\min(\Psi_{1}(\theta(y)),\Psi_{-1}(\theta(y)))}
        %    \\
        %    &\leq n \frac{\|\psi\|_{\infty}\sup_{y\in \bbR^d}|\theta_0(y)-\theta(y) |}{\inf_{\theta\in \Theta}\inf_{y\in \bbR^d}\min(\Psi_{1}(\theta(y)),\Psi_{-1}(\theta(y)))}
        %\|\max\left( \frac{\Psi_{1}(\theta_0(y))}{\Psi_{1}(\theta(y))},   \right)\|_{\infty}
    \end{align*}
    
    Note that  the derivative of the  exponent in the integrand  above with respect  to  $\theta(y)$   is 
    \begin{align} 
        \nonumber
        &\frac{\left(-  \lambda  \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{-\lambda-1} \psi(\theta(y)) +\lambda \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{-\lambda-1} \psi(\theta(y))  \right)}{ \left(   \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{-\lambda} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{-\lambda}   \right)  } 
        \\
        \nonumber
        &= \lambda \psi(\theta(y)) \frac{\left(-   \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{-\lambda-1} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{-\lambda-1}   \right) }{ \left(   \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{-\lambda} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{-\lambda}   \right)  } 
        \\
        \nonumber
        &= \lambda \frac{\psi(\theta(y))}{\Psi_{1}(\theta(y)) \Psi_{-1}(\theta(y))} \frac{\left(-   \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{\lambda+1} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{\lambda+1}   \right) }{ \left(   \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{\lambda} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{\lambda}   \right)  } 
        \\
        \nonumber
        &= \lambda  \frac{\left(-   \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{\lambda+1} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{\lambda+1}   \right) }{ \left(   \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{\lambda} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{\lambda}   \right)  } 
        \\
        \nonumber
        &= \lambda  \frac{\left(-   e^{-(\lambda+1)\theta(y)} + e^{-(1+\lambda)\theta_0(y)}\right) }{ \left(   e^{-\lambda\theta(y)} + e^{-(\lambda+1)\theta_0(y)}  \right) (1+e^{-\theta(y)})  } 
        \\
        \nonumber
        &= \lambda  \frac{ e^{-(1+\lambda)\theta_0(y)} \left(1 -   e^{-(\lambda+1)(\theta(y)-\theta_0(y))} \right) }{ \left(   e^{-\lambda\theta(y)} + e^{-(\lambda+1)\theta_0(y)}  \right) (1+e^{-\theta(y)})  } 
        \\
        \nonumber   
        &\leq \lambda  \frac{ (\lambda+1)  (\theta(y)-\theta_0(y))  }{ \left(   e^{-\lambda\theta(y)+(\lambda+1){\theta_0(y)}} + 1 \right) (1+e^{-\theta(y)})  } 
        \\
        &\leq \lambda  { (\lambda+1)  |\theta(y)-\theta_0(y)|  },
    \end{align}
    where in the fourth equality we used definition of the logistic function and the penultimate inequality follows from the well known inequality that $1-e^{-x}\leq x$. Consequently, using Taylor's theorem it follows that the exponent in the integrand is bounded above by $\lambda(\lambda+1)|\theta(y)-\theta_0(y)|^2 $  and thus by $\lambda(\lambda+1)\|\theta(y)-\theta_0(y)\|^2_{\infty} $. Therefore, 
    \begin{align*}
        D_{1+\lambda}(P_0^n\| P_{\theta}^n) &=  n \frac{1}{\lambda} \ln \int \left( \Psi_{1}(\theta_0(y))^{1+\lambda}\Psi_{1}(\theta(y))^{-\lambda} + \Psi_{-1}(\theta_0(y))^{1+\lambda}\Psi_{-1}(\theta(y))^{-\lambda}  \right) \nu(dy)
        \\
        &\leq n \frac{1}{\lambda} \ln \int e^{\lambda(\lambda+1)\|\theta(y)-\theta_0(y)\|^2_{\infty}} \nu(dy)
        \\
        &= n (\lambda+1)\|\theta(y)-\theta_0(y)\|^2_{\infty}.
    \end{align*}
    
    Now using the inequality for $C_3=16(\lambda+1)$ above observe that
    \begin{align}
        \nonumber
        \Pi(A_n)&=  \Pi(D_{1+\lambda} \left( P_0^n \| P_{\theta}^n \right) \leq C_3 n \e_n^2)
        \\
        \nonumber
        &\geq \Pi( n(\lambda+1)\|\theta(y)-\theta_0(y)\|^2_{\infty} \leq C_3 n\e_n^2  )
        \\
        &= \Pi( \|\theta(y)-\theta_0(y)\|_{\infty} \leq 4\e_n  )
        \geq  e^{-n\e_n^2}
    \end{align}
    and the  result follows from~\eqref{eq:renyiGP} of~Lemma~\ref{lem:GP}.
    %Now observe  that for $\lambda=2$ and two Bernoulli distribution $P$ and $Q$ with parameter $p$ and $Q$ respectively
    %\begin{align}
    %    \nonumber
    %D_{1+2}(P\| Q) &=\frac{1}{2} \ln \left( (p/q)^2 p + [(1-p)/(1-q)]^2 (1-p) \right)
    %\\
    %\nonumber
    %&=  \frac{1}{2} \ln \left( [1+(p-q)/q]^2 p + [1+(q-p)/(1-q)]^2 (1-p) \right)
    %\\
    %\nonumber
    %&= \frac{1}{2} \ln \left( [1+(p-q)^2/q^2 + 2(p-q)/q] p + [1+(q-p)^2/(1-q)^2+2(q-p)/(1-q)] (1-p) \right)
    %\\
    %\nonumber
    %&= \frac{1}{2} \ln \left( 1+(p-q)^2p/q^2  + (q-p)^2(1-p)/(1-q)^2 + 2(q-p) [   (1-p)/(1-q) - p/q ] \right)
    %\\
    %\nonumber
    %&= \frac{1}{2} \ln \left( 1+(p-q)^2p/q^2  + (q-p)^2(1-p)/(1-q)^2 + 2(q-p)^2/[q(1-q)] \right)
    %\\
    %\nonumber
    %&= \frac{1}{2} \ln \left( 1+(p-q)^2[ p/q^2  + (1-p)/(1-q)^2 + 2/[q(1-q)] ] \right)
    %\\
    %&\leq \frac{1}{2} \ln \left( 1+(p-q)^2[ 1/q^2  + 1/(1-q)^2 + 2/[q(1-q)] ] \right)
    %\\
    %&\leq \frac{1}{2} \ln \left( 1+(p-q)^2[ 1/q + 1/(1-q)]^2  \right)
    %\\
    %\nonumber
    %&= \frac{1}{2} \ln \left( 1+\left(\frac{(p-q)}{q(1-q)}\right)^2 \right)
    %\\
    %&\leq \frac{1}{2}(p-q)^2[ 3/\min(q,1-q)^2 ]
    %\end{align}
    %
    %Using the  above bound for $P=P_{0|y}$ and $Q=P_{\theta|y}$, we have
    %\begin{align}
    %    \nonumber
    %    D_{1+2}(P_0^n\| P_{\theta}^n) &=  n \frac{1}{2} \ln \int \left( \Psi_{1}(\theta_0(y))^{1+2}\Psi_{1}(\theta(y))^{-2} + \Psi_{-1}(\theta_0(y))^{1+2}\Psi_{-1}(\theta(y))^{-2}  \right) \nu(dy)
    %    \\
    %    \nonumber
    %    &= n \frac{1}{2} \ln \int e^{2 D_{1+2}(P_{0|y}\| P_{\theta|y})   } \nu(dy)
    %    \\
    %    \nonumber
    %    &\leq n \frac{1}{2} \ln \int e^{(\Psi_{1}(\theta_0(y))-\Psi_{1}(\theta(y)))^2[ 3/\min(\Psi_{1}(\theta(y)),\Psi_{-1}(\theta(y)))^2 ] } \nu(dy)
    %    \\
    %    \nonumber
    %     &\leq n \frac{1}{2} \ln \int e^{ \frac{3(\|\psi\|_{\infty}\sup_{y\in \bbR^d}|\theta_0(y)-\theta(y) |)^2}{\inf_{y\in \bbR^d} \min(\Psi_{1}(\theta(y)),\Psi_{-1}(\theta(y)))^2 } } \nu(dy)
    %     \\
    %     & = \frac{3n}{2} { \frac{\|\psi\|_{\infty}^2\|\theta_0(y)-\theta(y) \|_{\infty}^2}{\inf_{y\in \bbR^d} \min(\Psi_{1}(\theta(y)),\Psi_{-1}(\theta(y)))^2 } } .
    %       \end{align}
    
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:gp4}]
    Let us first analyze  the $\scKL$  divergence between the prior  distribution and variational family.
    Recall that  two Gaussian measures on infinite dimensional spaces  are either equivalent or singular.~\cite[Theorem 6.13]{Stuart2010} specify the condition  required  for the two Gaussian measures to be equivalent. In particular, note that  $\theta_0^J(\cdot)\in \text{Im}(\mathcal{C}^{1/2})$. Now observe that the covariance operator of $Q_n$ has eigenvalues ${\{\zeta^2_j\}_{j=1}^{J}}_{k=1}^{2^{jd}}$, therefore operator $S$ in the definition of $\mathcal{C}_q$ has eigenvalues ${\{1-\zeta^2_j/\mu_j^2\}_{j=1}^{J}}_{k=1}^{2^{jd}}$. For $\tau_j^2=2^{-2ja-jd}$ for any $a>0$,  $\sum_{j=1}^{J} 2^{jd} \left(\frac{n\e_n^2 2^{-2ja-jd} }{1+ n\e_n^2 2^{-2ja-jd} } \right)^2 = \sum_{j=1}^{J} 2^{-jd} \left(\frac{n\e_n^2 2^{-2ja} }{1+ n\e_n^2 2^{-2ja-jd} } \right)^2 <\infty$, therefore $S$ is an HS operator. 
    %    For any $h\in \bbH$, with $h_{j,k}=\langle  h,  \varphi_{j,k} \rangle $
    %    
    %    \begin{align}
    %        \frac{\langle h,\mathcal{C}_1h\rangle}{\langle h,\mathcal{C}_q h\rangle} = \frac{\sum_{j=1}^{ J} \sum_{k=1}^{2^{jd}}  \mu_j^2 h_{j,k} }{\sum_{j=1}^{ J}  \sum_{k=1}^{2^{jd}} \zeta_j^2 h_{j,k}} \leq 1.
    %        \end{align} 
    
    For any integer $J\leq J_{\alpha}$  define $\bar \theta_0^J = \int \theta_0^J(y) \nu(dy)$, where $\theta_0^J(\cdot)= \sum_{j=1}^{J} \sum_{k=1}^{2^{jd}} \theta_{0;j,k}  \vartheta_{j,k}(\cdot) $. Since, $\theta_0^J(\cdot)\in \text{Im}(\mathcal{C}^{1/2})$ and  $S$ is a  symmetric and HS operator, we invoke Theorem 5 in~\cite{quang2019}, to write  
    \begin{align*}
        \scKL(\mathcal{N}(\bar\theta_0^J,\mathcal{C}_q)\|\mathcal{N}(0,\mathcal{C})) &= \frac{1}{2}\| \mathcal{C}^{-1/2}\bar \theta_0^J \|^2 - \frac{1}{2} \log \det(I-S) + \frac{1}{2} tr(-S) ,
        \\
        &= \frac{1}{2}  \sum_{j=1}^{J} \sum_{k=1}^{2^{jd}} \frac{ \theta_{0;k,j}^2}{\mu_j^2} -\frac{1}{2} \log \prod_{j=1}^{J} \prod_{k=1}^{2^{jd}} (1-\kappa_{j}^2) -\frac{1}{2} \sum_{j=1}^{J} \sum_{k=1}^{2^{jd}} \kappa_j^2
        \\
        &= \frac{1}{2}  \sum_{j=1}^{J} \sum_{k=1}^{2^{jd}} \frac{ \theta_{0;k,j}^2}{\mu_j^2} -\frac{1}{2} \log \prod_{j=1}^{J}  (1-\kappa_{j}^2)^{2^{jd}} -\frac{1}{2} \sum_{j=1}^{J} 2^{jd} \kappa_j^2
        \\
        &= \frac{1}{2}  \sum_{j=1}^{J} \sum_{k=1}^{2^{jd}} \frac{ \theta_{0;k,j}^2}{\mu_j^2} -\frac{1}{2}   \sum_{j=1}^{J} {2^{jd}} \log (1-\kappa_{j}^2) -\frac{1}{2} \sum_{j=1}^{J} 2^{jd} \kappa_j^2.
    \end{align*}
    Now for $\mu_j 2^{jd/2}=2^{-ja}$, and using the definition of  Besov norm of $\theta_0$ denoted as $\|\theta_0\|^2_{\beta,\infty,\infty}$, and denoting $1-\kappa_j^2 = \frac{1}{1+n\e_n^2 \tau_j^2}$, we  have 
    \begin{align*}
        \scKL(\mathcal{N}(\bar\theta_0^J,\mathcal{C}_q)\|\mathcal{N}(0,\mathcal{C})) &\leq \frac{1}{2}  \sum_{j=1}^{J} {2^{j(2a-2\beta+d)}} \|\theta_0\|^2_{\beta,\infty,\infty}  -\frac{1}{2}   \sum_{j=1}^{J} {2^{jd}} \log (1-\kappa_{j}^2) -\frac{1}{2} \sum_{j=1}^{J} 2^{jd} \kappa_j^2
        \\
        &= \frac{1}{2}  \sum_{j=1}^{J} {2^{j(2a-2\beta+d)}} \|\theta_0\|^2_{\beta,\infty,\infty} - \frac{1}{2}  \sum_{j=1}^{J} 2^{jd} \left( \log (1-\kappa_{j}^2)    +  \kappa_j^2 \right)
        \\
        &= \frac{1}{2}  \sum_{j=1}^{J} {2^{j(2a-2\beta+d)}} \|\theta_0\|^2_{\beta,\infty,\infty} + \frac{1}{2}  \sum_{j=1}^{J} 2^{jd} \left( \log (1+n\e_n^2\tau_{j}^2)    - \frac{n\e_n^2\tau_j^2}{1+n\e_n^2\tau_j^2} \right)
        \\
        &\leq \frac{1}{2}  \sum_{j=1}^{J} {2^{j(2a-2\beta+d)}} \|\theta_0\|^2_{\beta,\infty,\infty} + \frac{1}{2}  \sum_{j=1}^{J} 2^{jd} \left(  n\e_n^2\tau_j^2 \right),
        %tr_{X}[(\mathcal{C}+\rho I)^{-1}(\mathcal{C}_q+\rho I)-I ]-\frac{1}{2} \log \det_{X}[(\mathcal{C}+\rho I)^{-1}(\mathcal{C}_q+\rho I)]     
    \end{align*}
    where the last inequality follows from the  fact that, $\log(1+x)-\frac{x}{1+x}\leq \frac{x^2}{1+x}\leq x$ for $x>0$.
    Substituting $\tau_j^2= 2^{-2ja-jd}$, we have
    \begin{align*}
        \frac{1}{n}\scKL(\mathcal{N}(\bar \theta_0^J,\mathcal{C}_q)\|\mathcal{N}(0,\mathcal{C})) &\leq \frac{1}{2n}  \sum_{j=1}^{J} {2^{j(2a-2\beta+d)}} \|\theta_0\|^2_{\beta,\infty,\infty} + \frac{\e_n^2}{2}  \sum_{j=1}^{J} 2^{-2ja} 
        \\
        & \leq \frac{\|\theta_0\|^2_{\beta,\infty,\infty}}{2n}  \sum_{j=1}^{J} {2^{j(2a-2\beta+d)}}  + \frac{2^{-2a}}{2}   \frac{1-2^{-2Ja} }{1-2^{-2a} } \e_n^2.
    \end{align*}
    
    The summation in the first term above is bounded by $\e_n^2$ as derived in~\cite[Theorem 4.5]{Zanten08}. Therefore,
    \begin{align}
        \frac{1}{n}\scKL(\mathcal{N}(\bar \theta_0^J,\mathcal{C}_q)\|\mathcal{N}(0,\mathcal{C})) 
        & \leq \max\left({\|\theta_0\|^2_{\beta,\infty,\infty}} ,   \frac{2^{-2a}-2^{-2Ja-2a} }{1-2^{-2a} }  \right)   \e_n^2.
        \label{eq:eqKL1}
    \end{align}
    
    Now consider the second term 
    \begin{align*}
        \frac{1}{n}\bbE_{Q_n} \scKL(P_0^n\| P_{\theta}^n) &=  \bbE_{Q_n} \int \left( \Psi_{1}(\theta_0(y)) \log\frac{\Psi_{1}(\theta_0(y))}{\Psi_{1}(\theta(y))} + \Psi_{-1}(\theta_0(y)) \log\frac{\Psi_{-1}(\theta_0(y))}{\Psi_{-1}(\theta(y))}  \right) \nu(dy)
        \\
        &\leq \bbE_{Q_n} \int \langle \theta(y)-\theta_0(y),\theta(y)-\theta_0(y)\rangle  \nu(dy)
        \\
        &= \bbE_{Q_n} \int \| \theta(y)-\theta_0^J(y) - ( \theta_0(y)-\theta_0^J(y))\|_2^2 \nu(dy)
        \\
        &= \bbE_{Q_n} \int \| \theta(y)-\theta_0^J(y)\|^2_2 + \| \theta_0(y)-\theta_0^J(y))\|_2^2 -2\langle \theta(y)-\theta_0^J(y),\theta_0(y)-\theta_0^J(y)\rangle  \nu(dy)
        \\
        &\leq \bbE_{Q_n} \int \| \theta(y)-\theta_0^J(y)\|^2_2  \nu(dy) + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty}
        \\
        &= \bbE_{Q_n} \int | \sum_{j=1}^{J} \sum_{k=1}^{2^{jd}} \zeta_j Z_{j,k} \vartheta_{j,k}(y)|^2  \nu(dy) + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty}
        \\
        &\leq \bbE_{Q_n} \sum_{j=1}^{J} \sum_{k=1}^{2^{jd}} \zeta_j^2 Z_{j,k}^2 \int  \vartheta_{j,k}(y)^2  \nu(dy) + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty} 
        \\
        &= \sum_{j=1}^{J} \sum_{k=1}^{2^{jd}} \zeta_j^2 \bbE_{Q_n}[Z_{j,k}^2] + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty}
        \\
        &=\sum_{j=1}^{J} \sum_{k=1}^{2^{jd}}   {\mu_j^2(1-\kappa_j^2)} + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty}
        \\
        &= \sum_{j=1}^{J} {2^{jd}}   \frac{\mu_j^2}{1+n\e_n^2\tau_j^2} + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty}
        \\
        &\leq   \frac{1}{n\e_n^2} \sum_{j=1}^{J}  \frac{2^{-2ja}}{  \tau_j^2}  + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty} 
        \\
        &= \frac{1}{n\e_n^2} \sum_{j=1}^{J} 2^{jd} + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty} 
        \\
        &=\frac{2^d}{n\e_n^2}  \frac{2^{dJ} -1 }{2^{d}-1}  + \| \theta_0(y)-\theta_0^J(y))\|^2_{\infty} 
        \\
        &\leq  \frac{2^d/(2^d-1)}{(\log n )^2}   + C' \e_n^2,
        %\leq \frac{1}{n\e_n^2}  \frac{n^{\frac{d}{2\alpha+d}} -1 }{2^{d}-1} 
        %\\
        %&= \frac{1}{n\e_n^2}  \frac{n^{\frac{d}{2\alpha+d}} -1 }{2^{d}-1} 
        %\\
        %&= n^{-2d/(2\a+d)} \frac{1-n^{-2(a-d)/(2\a+d) }}{1-2^{-2a}} 
    \end{align*}
    where in the second inequality we used the second assertion of Lemma 3.2~\cite{Zanten08} for logistic function, the fifth  inequality uses  the fact that $\theta(y)-\theta_0^J(y)$ is orthogonal to $\theta_0(y)-\theta_0^J(y)$. For any $a\leq \alpha$ fix $J=J_{\alpha}$ otherwise $J=J_a$, and then it is straight forward to check from the definition of $\e_n$ given in the assertion of the theorem that $(2^{dJ-1}/n\e_n^2) \leq (\log n)^{-2}$. The term  $\| \theta_0(y)-\theta_0^J(y))\|^2_{\infty} $ is also bounded by $C'\e_n^2$ as shown in the proof of Theorem 4.5 in~\cite{Zanten08}.
\end{proof}


\subsection{Eight-schools model (fixed n)}
In the Eight-schools problem~\citep{yao18a,kusmierczyk2019variational}, the objective was to study the effectiveness of the special coaching program for SAT exams, offered in 8 schools. Each school reported the treatment effect $y_i$ and its standard deviation $\sigma_i$, where $i\in \{1,2,3,\ldots,8\}$. The observations $\{y_i,\sigma_i\}_{i=1}^8$ are modeled using the following hierarchical Bayesian model :
\begin{enumerate}
    \item \textbf{Prior distributions:} $\mu \sim \mathcal{N}(\cdot |0,5)$ , $\tau \sim \text{half-Cauchy}(\cdot|0,5)$
    \item $\theta_i\sim \mathcal{N}(\cdot |\mu,\tau^2)$ and $y_i\sim \mathcal{N}(\cdot |\theta_i,\sigma_i^2)$ for each $i\in \{1,2,3,\ldots,8\}$
    % \item  for each $i\in \{1,2,3,\ldots,8\}$.
\end{enumerate}  

Consequently, the posterior distribution is defined as \[\pi_8(\mu,\tau,\{\theta_i\}_{i=1}^{8}|\{y_i,\sigma_i\}_{i=1}^8)\propto \mathcal{N}(\cdot |0,5) \text{half-Cauchy}(\cdot|0,5) \prod_{i=1}^{8} \mathcal{N}(\theta_i |\mu,\tau^2) \mathcal{N}(y_i |\theta_i,\sigma_i^2). \]


For a given treatment effect for eight schools $y\in \bbR^8$, the loss function is defined as:
\begin{align}
    \ell(y,a)= \sum_{i=1}^{8} l(y_i,a_i) , \text{ where } l(y_i,a_i) = \begin{cases} 
        0.2 ~|a_i-y_i|, ~~y_i\geq a_i\\
        (1-0.2)~|a_i-y_i|, ~~ y_i<a_i,
    \end{cases}
\end{align}
where the decision variable $a$ denotes the optimal effectiveness level.
%Note: The  loss function looks very similar to the newsvendor loss, with $h=0.2$ and $b=1-0.2$. Also notice that the loss function objective is only quantifies the difference in treatments ( or in means), which I think is standard in statistical quantitative studies.

%Since, the algorithm in Ku\'smierczyk et al. is developed to maximize utility, they find an $M$ (how?) and transform the loss function to utility as $u(y,a)= M-l(y,a)$, where as in our case we directly minimize the loss function. However, following Ku\'smierczyk et al., we also maximize the utility to study effect of $\gamma$ on learning risk-sensitive decision rule.

We define %$R(a,\theta)$
\[
%R(a,\theta) =  L(a,\theta),
%\text{ where } 
R(a,\theta)= \log \int p(y|\theta,\{\sigma_i\}_{i=1}^8) \ell(y,a) dy,  \]
$\theta \in \bbR^d$ and $\{\sigma_i\}_{i=1}^8$ is a sequence of covariates. 

Fix $n = 8$. For any $\epsilon > \epsilon_n $, $a\in  \sA$, and $\gamma > 0$, using  CS (H\'olders) inequality
\begin{align*}	
    \int_{\left\{{\gamma R(a,\theta )} > {C_4n \e_n^2} \right\} } & e^{\gamma R(a,\theta )} d\Pi(\theta) 
    \\
    &= \int_{\Theta}\Ind{\left\{{\gamma R(a,\theta )} > {C_4n \e_n^2} \right\} } e^{\gamma R(a,\theta )} d\Pi(\theta)
    \\
    &\leq  \left( \int_{\Theta}\Ind{\left\{{\gamma R(a,\theta )} > {C_4n \e_n^2} \right\} }  d\Pi(\theta) \right)^{1/2} \left( \int_{\Theta}  e^{2\gamma R(a,\theta )} d\Pi(\theta) \right)^{1/2} 
    \\
    &< e^{-{C_4n \e_n^2}}  \left(  \int_{\Theta}    \left(\sum_{i=1}^{8} \int_{}l(y,a_i )p(y|\theta_i,\sigma_i) dy\right)^{2\gamma} d\Pi(\theta) \right)
    \\
    &\leq e^{-{C_4n \e_n^2}} \sum_{i=1}^{8} \left(  \int_{\Theta_i}    \left( \int_{}l(y,a_i )p(y|\theta_i,\sigma_i) dy\right)^{2\gamma} \pi(\theta_i) d\theta_i \right)
    \\
    &= e^{-{C_4n \e_n^2}}  \left( \sum_{i=1}^{8} \int_{\Theta_i} \left[ { \int_{y\geq a_i}0.2|a_i-y| p(y|\theta_i,\sigma_i) dy}^{2\gamma}  + { \int_{y< a_i}0.8|y-a_i| p(y|\theta_i,\sigma_i) dy}^{2\gamma} \right] \pi(\theta_i) d\theta_i \right)
    \\
    &\leq 
    e^{-{C_4n \e_n^2}}  \left( \sum_{i=1}^{8} \int_{\Theta_i} \left[ { \int_{y\geq a_i}0.04(a_i-y)^2 p(y|\theta_i,\sigma_i) dy}^{\gamma}  + { \int_{y< a_i}0.16(y-a_i)^2 p(y|\theta_i,\sigma_i) dy}^{\gamma} \right] \pi(\theta_i) d\theta_i \right)
    \\
    &\leq 
    e^{-{C_4n \e_n^2}}  \left( \sum_{i=1}^{8}  [(0.2\sigma_i)^{2\gamma} + (0.8\sigma_i)^{2\gamma}] + \sum_{i=1}^{8}  \int_{\Theta_i} \left[ (0.2(a_i-\theta_i))^{2\gamma} + (0.8(a_i-\theta_i))^{2\gamma} \right] \pi(\theta_i) d\theta_i \right)
    \\
    &\leq 
    e^{-{C_4n \e_n^2}}  \left( \sum_{i=1}^{8}  [2(0.8\sigma_i)^{2\gamma} ] + \sum_{i=1}^{8}  \int_{\Theta_i} \left[ 2(0.8|a_i-\theta_i|)^{2\gamma} \right] \pi(\theta_i) d\theta_i \right)
    \\
    &\leq 
    e^{-{C_4n \e_n^2}}  \left( \sum_{i=1}^{8}  \left[ 2(0.8\sigma_i)^{2\gamma}+ 2(0.8a_i)^{2\gamma} \right] + 2(0.8)^{2\gamma} \sum_{i=1}^{8}  \int_{\Theta_i}  |\theta_i|^{2\gamma}  \pi(\theta_i) d\theta_i  \right)
    \\
    &\leq 
    e^{-{C_4n \e_n^2}}  \left( \sum_{i=1}^{8}  \left[ 2(0.8\sigma_i)^{2\gamma}+ 2(0.8a_i)^{2\gamma} \right] + 2(0.8)^{2\gamma} \sum_{i=1}^{8} \left( |\mu|^{2\gamma}+ \int_{\Theta_i} |\theta_i-\mu|^{2\gamma}  \pi(\theta_i) d\theta_i \right) \right)
    \\
    &= e^{-{C_4n \e_n^2}}  \left( \sum_{i=1}^{8}  \left[ 2(0.8\sigma_i)^{2\gamma}+ 2(0.8a_i)^{2\gamma} \right] + 2(0.8)^{2\gamma} \sum_{i=1}^{8} \left( |\mu|^{2\gamma}+ \tau^{2\gamma}\frac{2^{\gamma}\Gamma(\frac{2\gamma+1}{2})}{\sqrt{\pi}} \right) \right)
    %\\
    %&= e^{-{C_4n \e_n^2} + 16\gamma \max{\sigma_i}}  \left( \prod_{i=1}^{8} \int_{\Theta_i}   e^{2\gamma|a_i-\theta_i| } \pi(\theta_i) d\theta_i \right)
    %\\
    %&=e^{-{C_4n \e_n^2} + 16\gamma \max{(\sigma_i+|a_i|)}}  \left( \prod_{i=1}^{8} \int_{\Theta_i}   e^{2\gamma|\theta_i| } \sN(\theta_i;\mu,\tau^2) d\theta_i \right)
    %\exp(-C_5 n\e_n^2),
\end{align*}
%where $C_4$ and  $C_5$ are positive constants.
%\begin{align*}	
%    \int_{\left\{{\gamma R(a,\theta )} > {C_4n \e_n^2} \right\} } & e^{\gamma R(a,\theta )} d\Pi(\theta) 
%    \\
%    &= \int_{\Theta}\Ind{\left\{{\gamma R(a,\theta )} > {C_4n \e_n^2} \right\} } e^{\gamma R(a,\theta )} d\Pi(\theta)
%    \\
%    &\leq  \left( \int_{\Theta}\Ind{\left\{{\gamma R(a,\theta )} > {C_4n \e_n^2} \right\} }  d\Pi(\theta) \right)^{1/2} \left( \int_{\Theta}  e^{2\gamma R(a,\theta )} d\Pi(\theta) \right)^{1/2} 
%    \\
%    &< e^{-{C_4n \e_n^2}}  \left( \prod_{i=1}^{8} \int_{\Theta_i}  e^{2\gamma \int_{}l(y,a_i )p(y|\theta_i,\sigma_i) dy} \pi(\theta_i) d\theta_i \right)
%    \\
%    &= e^{-{C_4n \e_n^2}}  \left( \prod_{i=1}^{8} \int_{\Theta_i}  e^{2\gamma \int_{y\geq a_i}0.2|a_i-y| p(y|\theta_i,\sigma_i) dy} e^{2\gamma \int_{y< a_i}0.8|y-a_i| p(y|\theta_i,\sigma_i) dy} \pi(\theta_i) d\theta_i \right)
%    \\
%    &\leq e^{-{C_4n \e_n^2}}  \left( \prod_{i=1}^{8} \int_{\Theta_i}  e^{2\gamma\sigma_i} e^{2\gamma|a_i-\theta_i| } \pi(\theta_i) d\theta_i \right)
%    \\
%    &= e^{-{C_4n \e_n^2} + 16\gamma \max{\sigma_i}}  \left( \prod_{i=1}^{8} \int_{\Theta_i}   e^{2\gamma|a_i-\theta_i| } \pi(\theta_i) d\theta_i \right)
%    \\
%    &=e^{-{C_4n \e_n^2} + 16\gamma \max{(\sigma_i+|a_i|)}}  \left( \prod_{i=1}^{8} \int_{\Theta_i}   e^{2\gamma|\theta_i| } \sN(\theta_i;\mu,\tau^2) d\theta_i \right)
%    %\exp(-C_5 n\e_n^2),
%\end{align*}

%Therefore, the ELBO joint-optimization problem in Ku\'smierczyk et al. is defined as
%\begin{align} 
%    \nonumber 
%    \max_{a\in\sA}\max_{q \in \mathcal M} \left\{ \mathbb
%    E_q[R(a,\theta)] - 
%    \text{KL}(q||\pi_8) \right\} 
%\end{align}

Notice that, it corresponds to choosing $\gamma=1$ in our RSVB formulation.
%, but using $\log-$utility as $R(a,\theta)$. 
Now for any $\gamma>0$, RSVB  joint-optimization problem is defined as
\begin{align} \min_{a\in\sA}\max_{Q \in \sQ} \left\{ \mathbb
    E_q[R(a,\theta)] - 
    \frac{1}{\gamma}\text{KL}(q||\pi_8) \right\}.
    %&= \frac{1}{\gamma}\min_{a\in\sA}\max_{q \in \mathcal M} \left\{ \mathbb
    %E_q[\log \pi_8 U(a,\theta)^\gamma - 
    %\log q] \right\}  
\end{align}

Following~\cite{kusmierczyk2019variational}, we fix the variational family $\sQ$ to be the mean-field variational family, that is 
\begin{align}
    q_{\Lambda}(\mu,\tau,{\theta_1}_{i=1}^{8})= \sN_{\mu}(\cdot|\lambda_{9})\sN_{\tau}(\cdot|\lambda_{10})\prod_{i=1}^{8}\sN_{\theta_i}(|\lambda_{i}),
\end{align}
where $\Lambda=\{\lambda_1,\lambda_2,\ldots,\lambda_{10}\}$, $\lambda_{i}$ is the mean and variance parameter for each Gaussian distribution. 

Analogous to~\cite{kusmierczyk2019variational}, we measure the performance of the RSVB method using the metric called \textit{empirical risk reduction} (ERR) ,
\[ \mathcal{I}= {\mathcal{ER}_{VI}- \mathcal{ER}_{RSVB(\gamma)}}%{\mathcal{ER}_{VI}}
,\text{ where }, \mathcal{ER}_{alg}= \frac{1}{N_Y} \sum_{j=1}^{N_Y}l(y_j^{test},a_{alg}) ,\]
where $\mathcal{ER}_{alg}$ denote the empirical risk evaluated at the decision rule $a^{alg}$ obtained using method $alg\in \{\text{VI,RSVB($\gamma$)}\}$ for various values of $\gamma$, and $N_Y$ is the size of the test data $\{y_j^{test}\}$. Note that ERR is the empirical approximation of the difference of optimality gap between the $VI$ and $RSVB(\gamma)$ approach. 

We modified the  experiments in ~\cite{kusmierczyk2019variational} by introducing $\gamma=\{5,2.5,1,0.5\}= \{0.2^{-1},0.4^{-1},1^{-1},2^{-1}\}$ 
%0.6^{-1},0.8^{-1} 1.66,1.25
and obtain the results as summarized in Figure~\ref{fig:fig2} and~\ref{fig:fig3}.. In Figure~\ref{fig:fig2}, observe that as $\gamma$ increases the ERR also increases, which implies that the decisions are more risk averse as empirical loss using RSVB decision rule decreases as $\gamma$ increases. Also observe form Figure~\ref{fig:fig3} that, as $\gamma $ increases the RSVB posterior approaches to the true posterior and the variance of the approximate posterior also reduces.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/ERR_Lossmin.png}
    
    \caption{Empirical risk reduction (as defined in Ku\'smierczyk et al.) plot for different level of risk sensitivity. }\label{fig:fig2}
\end{figure}

\begin{figure}[H]
    \centering
    
    \begin{subfigure}[b]{0.9\textwidth}
        \includegraphics[width=\textwidth]{Figures/Posterior_LossMin.png}
        \caption{$\{\theta_1,\tau\}$}
        %\label{fig:f1}
    \end{subfigure}
    %    %\hfill
    %    \begin{subfigure}[b]{0.49\textwidth}
    %        \includegraphics[trim={0 0 6.5cm 1cm},clip,width=\textwidth]{Figures/8schools_loss_iterations_Post_T2tau.png}
    %        \caption{$\{\theta_2,\tau\}$}
    %        %       %\label{fig:f2}
    %    \end{subfigure}
    %    \begin{subfigure}[b]{0.49\textwidth}
    %        \includegraphics[trim={0 0 6.5cm 1cm},clip,width=\textwidth]{Figures/8schools_loss_iterations_Post_T3tau.png}
    %        \caption{$\{\theta_3,\tau\}$}
    %        
    %        %       %\label{fig:f2}
    %    \end{subfigure}
    
    %    \begin{subfigure}[b]{0.49\textwidth}
    %        \includegraphics[trim={0 0 6.5cm 1cm},clip,width=\textwidth]{Figures/8schools_loss_iterations_Post_T6tau.png}
    %        \caption{$\{\theta_6,\tau\}$}
    %    \end{subfigure}
    %    \begin{subfigure}[b]{0.49\textwidth}
    %        \includegraphics[trim={0 0 6.5cm 1cm},clip,width=\textwidth]{Figures/8schools_loss_iterations_Post_T7tau.png}
    %        \caption{$\{\theta_7,\tau\}$}
    %    \end{subfigure}
    
    \caption{Joint posterior distribution of $\{\theta_i,\tau\}$, plot for different level of risk sensitivity. }\label{fig:fig3}
\end{figure}
